Spectral Methods for Data Science: A Statistical Perspective

Spectral methods have emerged as a simple yet surprisingly effective approach for extracting information from massive, noisy and incomplete data. In a nutshell, spectral methods refer to a collection of algorithms built upon the eigenvalues (resp. singular values) and eigenvectors (resp. singular vectors) of some properly designed matrices constructed from data. A diverse array of applications have been found in machine learning, data science, and signal processing. Due to their simplicity and effectiveness, spectral methods are not only used as a stand-alone estimator, but also frequently employed to initialize other more sophisticated algorithms to improve performance. While the studies of spectral methods can be traced back to classical matrix perturbation theory and methods of moments, the past decade has witnessed tremendous theoretical advances in demystifying their efficacy through the lens of statistical modeling, with the aid of non-asymptotic random matrix theory. This monograph aims to present a systematic, comprehensive, yet accessible introduction to spectral methods from a modern statistical perspective, highlighting their algorithmic implications in diverse large-scale applications. In particular, our exposition gravitates around several central questions that span various applications: how to characterize the sample efficiency of spectral methods in reaching a target level of statistical accuracy, and how to assess their stability in the face of random noise, missing data, and adversarial corruptions? In addition to conventional $\ell_2$ perturbation analysis, we present a systematic $\ell_{\infty}$ and $\ell_{2,\infty}$ perturbation theory for eigenspace and singular subspaces, which has only recently become available owing to a powerful "leave-one-out" analysis framework.

==> MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{Toyota Technological Institute}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Northeastern University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Amazon}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{Yale}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{KU Leuven}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Microsoft Research}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Computational Optimal Transport}\\
Gabriel Peyre and Marco Cuturi\\
ISBN: 978-1-68083-550-2\\
\\
\noindent \textit{An Introduction to Deep Reinforcement Learning}\\
Vincent Francois-Lavet, Peter Henderson, Riashat Islam,\\ Marc G. Bellemare and Joelle Pineau \\
ISBN: 978-1-68083-538-0\\
\\
\noindent \textit{An Introduction to Wishart Matrix Moments}\\
Adrian N. Bishop, Pierre Del Moral and Angele Niclas \\
ISBN: 978-1-68083-506-9\\
\\
\noindent \textit{A Tutorial on Thompson Sampling}\\
Daniel J. Russo, Benjamin Van Roy, Abbas Kazerouni, Ian Osband\\ and Zheng Wen\\
ISBN: 978-1-68083-470-3\\

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> chapters/old_notes/entrywise_bound.tex <==
For notational convenience, we first define
\begin{equation}
\bm{Y}\coloneqq\bm{M}\bm{U}^{\star}\big(\bm{\Lambda}^{\star}\big)^{-1}=\bm{U}^{\star}+\bm{E}\bm{U}^{\star}\big(\bm{\Lambda}^{\star}\big)^{-1},\label{eq:defn-Y-MULambda}
\end{equation}
which clearly satisfies
\begin{align*}
\bm{Y}\bm{\Lambda}^{\star}\bm{Y}^{\top} & =\Big(\bm{U}^{\star}+\bm{E}\bm{U}^{\star}\big(\bm{\Lambda}^{\star}\big)^{-1}\Big)\bm{\Lambda}^{\star}\Big(\bm{U}^{\star}+\bm{E}\bm{U}^{\star}\big(\bm{\Lambda}^{\star}\big)^{-1}\Big)^{\top}\\
 & =\bm{M}^{\star}+\bm{E}\bm{U}^{\star}\bm{U}^{\star\top}+\bm{U}^{\star}\bm{U}^{\star\top}\bm{E}+\bm{E}\bm{U}^{\star}\big(\bm{\Lambda}^{\star}\big)^{-1}\bm{U}^{\star\top}\bm{E}.
\end{align*}
In words, $\bm{Y}\bm{\Lambda}^{\star}\bm{Y}^{\top}$ can be viewed
as the ground truth $\bm{M}^{\star}=\bm{U}^{\star}\bm{\Lambda}^{\star}\bm{U}^{\star\top}$
corrupted by some simple functions of $\bm{E}$, and might often be
viewed as a surrogate of $\bm{M}^{\star}$. In order to study the
estimation error of $\bm{U}\bm{\Lambda}\bm{U}^{\top}$, the key step
lies in the following observation
%
\begin{align}
 & \big\|\bm{U}\bm{\Lambda}\bm{U}^{\top}-\bm{Y}\bm{\Lambda}^{\star}\bm{Y}^{\top}\big\|_{\infty}\leq\underset{\eqqcolon\mathcal{\gamma}_{1}}{\underbrace{\big\|\bm{U}\big(\bm{\Lambda}-\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}\big)\bm{U}^{\top}\big\|_{\infty}}}\nonumber \\
 & \quad\quad\quad\quad+
	\underset{\eqqcolon\gamma_{2}}{\underbrace{\big\|\bm{U}\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}\bm{U}^{\top}-\bm{Y}\bm{\Lambda}^{\star}\bm{Y}^{\top}\big\|_{\infty}}},
\label{eq:ULambdaU-YLambdaY-decompose}
\end{align}
%
thus leaving us with two terms to handle. 





\subsubsection{Step 2: bounding $\gamma_1$}

Regarding the first term $\big\|\bm{U}\big(\bm{\Lambda}-\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}\big)\bm{U}^{\top}\big\|_{\infty}$,
it is seen that
%
\begin{align}
\gamma_{1} & \leq\big\|\bm{U}\big\|_{\infty}^{2}\big\|\bm{\Lambda}-\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}\big\|\leq\frac{4\mu r}{n}\big\|\bm{\Lambda}-\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}\big\|.
	\label{eq:gamma1-UB-12345}
\end{align}
%
Here, we have made use of the fact that
\[
\big\|\bm{U}\big\|_{\infty}=\big\|\bm{U}\mathsf{sgn}(\bm{H})\big\|_{\infty}\leq\big\|\bm{U}^{\star}\big\|_{\infty}+\big\|\bm{U}\mathsf{sgn}(\bm{H})-\bm{U}^{\star}\big\|_{\infty}\leq2\sqrt{\mu r/n},
\]
where the last inequality relies on (\ref{eq:UsgnH-Ustar-bound-theorem-general})
and the assumption $\sigma\sqrt{n}(\kappa+\sqrt{\log n})\leq c_{1}\lambda_{r}^{\star}$
for some sufficiently small constant $c_{1}>0$. 




It then boils down to bounding $\|\bm{\Lambda}-\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}\|$.
Towards this, it is  seen from the identity (\ref{eq:HLambda-Lambda-H-connection})
and the definition $\bm{H}=\bm{U}^{\top}\bm{U}^{\star}$ that
%
\begin{align*}
\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}-\bm{\Lambda} & =\bm{\Lambda}\bm{H}\bm{H}^{\top}-\bm{U}^{\top}\bm{E}\bm{U}^{\star}\bm{H}^{\top}-\bm{\Lambda},
\end{align*}
%
which together with the triangle inequality gives
%
\begin{align}
\big\|\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}-\bm{\Lambda}\big\| & \leq\big\|\bm{\Lambda}\big(\bm{H}\bm{H}^{\top}-\bm{I}\big)\big\|+\big\|\bm{U}^{\top}\bm{E}\bm{U}^{\star}\bm{H}^{\top}\big\|.
	\label{eq:HLambda-H-ambda-bound-2terms}
\end{align}
%


Regarding the first term on the right-hand side of (\ref{eq:HLambda-H-ambda-bound-2terms}), we make the observation that
%
\[
\|\bm{H}\bm{H}^{\top}-\bm{I}\|=\|\cos^{2}\bm{\Theta}-\bm{I}\|=\|\sin^{2}\bm{\Theta}\|\leq\frac{2c_{2}\sigma^{2}n}{(\lambda_{r}^{\star})^{2}},
\]
%
where, as usual, $\bm{\Theta}$ denotes a diagonal matrix composed
of the principal angles between $\bm{U}$ and $\bm{U}^{\star}$. This
combined with Weyl's inequality and Lemma \ref{lem:preliminary-result-general-iid} leads to
%
\begin{align}
\|\bm{\Lambda}(\bm{H}\bm{H}^{\top}-\bm{I})\| & \leq\|\bm{\Lambda}\|\,\|\bm{H}\bm{H}^{\top}-\bm{I}\|\leq(\|\bm{\Lambda}^{\star}\|+\|\bm{E}\|)\,\|\bm{H}\bm{H}^{\top}-\bm{I}\|\nonumber \\
 & \leq\big(\big|\lambda_{1}^{\star}\big|+c_{2}\sigma\sqrt{n}\big)\frac{2c_{2}\sigma^{2}n}{(\lambda_{r}^{\star})^{2}}\leq\frac{4c_{2}\kappa\sigma^{2}n}{\lambda_{r}^{\star}},
\label{eq:Lambda-HHT-I-bound}
\end{align}
%
provided that $c_{2}\sigma\sqrt{n}\leq\lambda_{r}^{\star}\leq|\lambda_{1}^{\star}|$.



When it comes to the second term on the right-hand side of (\ref{eq:HLambda-H-ambda-bound-2terms}),
let us introduce an orthornormal matrix $\bm{R}\coloneqq\arg\min_{\bm{Q}\in\mathcal{O}^{r\times r}}\|\bm{U}\bm{Q}-\bm{U}^{\star}\|$,
which allows us to derive
%
\begin{align}
\big\|\bm{U}^{\top}\bm{E}\bm{U}^{\star}\bm{H}^{\top}\big\| & \leq\big\|\bm{U}^{\top}\bm{E}\bm{U}^{\star}\big\|=\big\|\bm{R}^{\top}\bm{U}^{\top}\bm{E}\bm{U}^{\star}\big\| \notag\\
 & \leq\big\|\bm{U}^{\star\top}\bm{E}\bm{U}^{\star}\big\|+\big\|\big(\bm{U}\bm{R}-\bm{U}^{\star}\big)^{\top}\bm{E}\bm{U}^{\star}\big\| \notag\\
	& \leq\big\|\bm{U}^{\star\top}\bm{E}\bm{U}^{\star}\big\|+\|\bm{E}\|\,\mathsf{dist}\big(\bm{U},\bm{U}^{\star}\big). \label{eq:Utop-E-U-H-bound12}
\end{align}
%
Here, the first inequality holds since $\|\bm{H}\|=\|\bm{U}^{\top}\bm{U}^{\star}\|\leq1$,
the second inequality relies on Remark \ref{remark:AH-norm-bound},
while the last line follows since $\|\bm{U}^{\star}\|=1$ and $\|\bm{U}\bm{R}-\bm{U}^{\star}\|=\mathsf{dist}(\bm{U},\bm{U}^{\star})$. 
We now claim that with probability at least $1-2n^{-7}$,
%
\begin{equation}
\|\bm{U}^{\star\top}\bm{E}\bm{U}^{\star}\|\leq(6+c_{\mathsf{b}})\sigma\sqrt{r\log n}.
	\label{eq:claim-Utop-E-Ustar-spectral-norm}
\end{equation}
%
If this claim were valid, then we could continue the derivation (\ref{eq:Utop-E-U-H-bound12}) and invoke Lemma \ref{lem:preliminary-result-general-iid} to arrive at
%
\begin{equation}
\big\|\bm{U}^{\top}\bm{E}\bm{U}^{\star}\bm{H}^{\top}\big\|\leq(6+c_{\mathsf{b}})\sigma\sqrt{r\log n}+\frac{2c_{2}^{2}\sigma^{2}n}{\lambda_{r}^{\star}}.
	\label{eq:UB-UEUHtop-UB1}
\end{equation}
%

To finish up, substituting \eqref{eq:Lambda-HHT-I-bound} and \eqref{eq:UB-UEUHtop-UB1} into \eqref{eq:HLambda-H-ambda-bound-2terms} yields
%
\[
\big\|\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}-\bm{\Lambda}\big\|\leq\frac{6c_{2}\kappa\sigma^{2}n}{\lambda_{r}^{\star}}+7\sigma\sqrt{r\log n} , 
\]
%
provided  that $c_2\leq 1$ and $c_{\mathsf{b}}\leq 1$.  
This combined with \eqref{eq:gamma1-UB-12345} gives
%
\begin{equation}
\gamma_{1}\leq\frac{24c_{2}\sigma^{2} \kappa\mu r}{\lambda_{r}^{\star}}+\frac{28\sigma\mu\sqrt{r^{3}\log n}}{n}.
\label{eq:gamma1-UB-2346}
\end{equation}
%



\subsubsection{Step 3: bounding $\gamma_2$}

Before proceeding, we first gather a simple bound on $\|\bm{Y}\|_{2,\infty}$.
It is seen from the definition of $\bm{Y}$ that
\begin{align}
\|\bm{Y}\|_{2,\infty} & \leq\big\|\bm{U}^{\star}\big\|_{2,\infty}+\big\|\bm{E}\bm{U}^{\star}\big(\bm{\Lambda}^{\star}\big)^{-1}\big\|_{2,\infty}\leq\sqrt{\frac{\mu r}{n}}+\frac{\big\|\bm{E}\bm{U}^{\star}\big\|_{2,\infty}}{\lambda_{r}^{\star}}\nonumber \\
 & \overset{(\mathrm{i})}{\leq}\sqrt{\frac{\mu r}{n}}+\frac{10\sigma\sqrt{r\log n}}{\lambda_{r}^{\star}}\overset{(\mathrm{ii})}{\leq}2\sqrt{\frac{\mu r}{n}},\label{eq:Y-2-inf-bound-123}
\end{align}
where (i) comes from (\ref{eq:EU-2-inf-bound-general}) and the assumption
$c_{\mathsf{b}}\leq1$, and (ii) is valid as long as $10\sigma\sqrt{n\log n}\leq\lambda_{r}^{\star}$.
In addition, it follows from (\ref{eq:UH-MUstar-Lambda-star-2inf})
that
\begin{align}
\big\|\bm{U}\bm{H}-\bm{Y}\big\|_{2,\infty} & \lesssim\frac{\sigma\kappa\sqrt{\mu r}}{\lambda_{r}^{\star}}+\frac{c_{\mathsf{b}}\sigma^{2}\sqrt{rn}\log n}{\big(\lambda_{r}^{\star}\big)^{2}}\lesssim\frac{\sigma\kappa\sqrt{\mu r\log n}}{\lambda_{r}^{\star}},\label{eq:UH-MUstar-Lambda-star-2inf-1}
\end{align}
with the proviso that $\sigma\sqrt{n\log n}\lesssim\lambda_{r}^{\star}$.





Recognizing the basic decomposition
%
\begin{align*}
\bm{U}\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}\bm{U}^{\top}-\bm{Y}\bm{\Lambda}^{\star}\bm{Y}^{\top} & =(\bm{U}\bm{H}-\bm{Y})\bm{\Lambda}^{\star}\bm{Y}^{\top}+\bm{Y}\bm{\Lambda}^{\star}(\bm{U}\bm{H}-\bm{Y})^{\top}\\
 & \quad+(\bm{U}\bm{H}-\bm{Y})\bm{\Lambda}^{\star}(\bm{U}\bm{H}-\bm{Y})^{\top},
\end{align*}
%
we can control each of these three terms separately.  
Firstly, observe that
\begin{align*}
\big\|\bm{A}_{1}\big\|_{\infty} & \leq\|\bm{U}\bm{H}-\bm{Y}\|_{2,\infty}\big\|\bm{Y}\big\|_{2,\infty}\big\|\bm{\Lambda}^{\star}\big\|\\
 & \lesssim\big|\lambda_{1}^{\star}\big|\sqrt{\frac{\mu r}{n}}\frac{\sigma\kappa\sqrt{\mu r\log n}}{\lambda_{r}^{\star}}\asymp\sigma\kappa^{2}\mu r\sqrt{\frac{\log n}{n}},
\end{align*}
where we have made use of (\ref{eq:Y-2-inf-bound-123}) and (\ref{eq:UH-MUstar-Lambda-star-2inf-1}).
Similarly,
\begin{align*}
\big\|\bm{A}_{2}\big\|_{\infty} & \leq\|\bm{U}\bm{H}-\bm{Y}\|_{2,\infty}^{2}\big\|\bm{\Lambda}^{\star}\big\|\lesssim\big|\lambda_{1}^{\star}\big|\frac{\sigma^{2}\kappa^{2}\mu r\log n}{\big(\lambda_{r}^{\star}\big)^{2}}\\
 & \asymp\frac{\sigma^{2}\kappa^{3}\mu r\log n}{\lambda_{r}^{\star}}\lesssim\sigma\kappa^{2}\mu r\sqrt{\frac{\log n}{n}},
\end{align*}
provided that $\sigma\kappa\sqrt{n\log n}\lesssim\lambda_{r}^{\star}$.
Consequently,
%
\begin{align*}
% \big\|\bm{U}\bm{H}\bm{\Lambda}^{\star}\bm{H}^{\top}\bm{U}^{\top}-\bm{Y}\bm{\Lambda}^{\star}\bm{Y}^{\top}\big\|_{\infty} 
\gamma_2 & \leq2\big\|\bm{A}_{1}\big\|_{\infty}+\big\|\bm{A}_{2}\big\|_{\infty}\lesssim\sigma\kappa^{2}\mu r\sqrt{\frac{\log n}{n}}.
\end{align*}



\subsubsection{Step 4: putting all this together}

Combining the above bounds, we demonstrate that
%
\begin{align}
	& \big\|\bm{U}\bm{\Lambda}\bm{U}^{\top}-\bm{Y}\bm{\Lambda}^{\star}\bm{Y}^{\top}\big\|_{\infty} 
	\leq\gamma_{1}+\gamma_{2} \notag\\
& \lesssim\sigma\kappa^{2}\mu r\sqrt{\frac{\log n}{n}}+\frac{\kappa\mu r\sigma^{2}}{\lambda_{r}^{\star}}+\frac{\sigma\mu r\sqrt{r\log n}}{n} 
  \asymp\sigma\kappa^{2}\mu r\sqrt{\frac{\log n}{n}}.
\end{align}
%




\begin{proof}[Proof of the claim \eqref{eq:claim-Utop-E-Ustar-spectral-norm}]

% Preview source code for paragraph 3

Let us start by expressing $\bm{U}^{\star\top}\bm{E}\bm{U}^{\star}$
as a sum of independent random matrices as follows
%
\[
\bm{U}^{\star\top}\bm{E}\bm{U}^{\star}=\sum_{i,j:\,i>j}E_{i,j}\Big\{\big(\bm{U}_{i,\cdot}^{\star}\big)^{\top}\bm{U}_{j,\cdot}^{\star}+\big(\bm{U}_{j,\cdot}^{\star}\big)^{\top}\bm{U}_{i,\cdot}^{\star}\Big\}\eqqcolon\sum_{i,j:\,i>j}\bm{Z}_{i,j}.
\]
%
From the elementary inequality $(\bm{A}+\bm{A}^{\top})^{2}\preceq2\bm{A}\bm{A}^{\top}+2\bm{A}^{\top}\bm{A}$, we have 
%
\begin{align*}
\mathbb{E}\big[\bm{Z}_{i,j}^{2}\big] & \preceq\sigma^{2}\Big\{\big(\bm{U}_{i,\cdot}^{\star}\big)^{\top}\bm{U}_{j,\cdot}^{\star}+\big(\bm{U}_{j,\cdot}^{\star}\big)^{\top}\bm{U}_{i,\cdot}^{\star}\Big\}\Big\{\big(\bm{U}_{i,\cdot}^{\star}\big)^{\top}\bm{U}_{j,\cdot}^{\star}+\big(\bm{U}_{j,\cdot}^{\star}\big)^{\top}\bm{U}_{i,\cdot}^{\star}\Big\}^{\top}\\
 & \preceq2\sigma^{2}\Big\{\big\|\bm{U}_{j,\cdot}^{\star}\big\|_{2}^{2}\big(\bm{U}_{i,\cdot}^{\star}\big)^{\top}\bm{U}_{i,\cdot}^{\star}+\big\|\bm{U}_{i,\cdot}^{\star}\big\|_{2}^{2}\big(\bm{U}_{j,\cdot}^{\star}\big)^{\top}\bm{U}_{j,\cdot}^{\star}\Big\},
\end{align*}
%
thus indicating that
%
\begin{align*}
v & =\Big\|\sum_{i,j:i>j}\mathbb{E}\big[\bm{Z}_{i,j}^{2}\big]\Big\|\leq2\sigma^{2}\Big\|\sum_{i=1}^{n}\sum_{j=1}^{n}\big\|\bm{U}_{j,\cdot}^{\star}\big\|_{2}^{2}\big(\bm{U}_{i,\cdot}^{\star}\big)^{\top}\bm{U}_{i,\cdot}^{\star}\Big\|\\
 & =2\sigma^{2}\|\bm{U}^{\star}\|_{\mathrm{F}}^{2}\Big\|\sum_{i,j}\big(\bm{U}_{i,\cdot}^{\star}\big)^{\top}\bm{U}_{i,\cdot}^{\star}\Big\|=2\sigma^{2}r\Big\|\bm{U}^{\star\top}\bm{U}^{\star}\Big\|=2\sigma^{2}r.
\end{align*}
%
In addition, each matrix $\bm{Z}_{i,j}$ can be bounded in size by
%
\[
\max_{i,j}\|\bm{Z}_{i,j}\|\leq2\max_{i,j}\big|E_{i,j}\big|\max_{i,j}\big\|\bm{U}_{i,\cdot}^{\star}\big\|_{2}\big\|\bm{U}_{j,\cdot}^{\star}\big\|_{2}\leq2B\frac{\mu r}{n}\eqqcolon L.
\]
%
Apply the matrix Bernstein inequality (see Corollary \ref{thm:matrix-Bernstein-friendly}) to reach
%
\begin{align*}
\big\|\bm{U}^{\star\top}\bm{E}\bm{U}^{\star}\big\| & \leq4\sqrt{v\log n}+6L\log n\leq\sigma\sqrt{32r\log n}+2B\frac{\mu r\log n}{n}\\
 & \leq(6+c_{\mathsf{b}})\sigma\sqrt{r\log n}
\end{align*}
%
with probability exceeding $1-2n^{-7}.$ Here, the last line holds since
%
\[
B\frac{\mu r\log n}{n}\leq c_{\mathsf{b}}\sigma\sqrt{\frac{n}{\mu\log n}}\cdot\frac{\mu r\log n}{n}=c_{\mathsf{b}}\sigma\sqrt{r\log n}\sqrt{\frac{\mu r}{n}}\leq c_{\mathsf{b}}\sigma\sqrt{r\log n},
\]
%
which relies on the assumption (\ref{eq:assumption-B-sigma}) and the fact $\mu\leq n/r$. 
%
\end{proof}




==> chapters/old_notes/generalization.tex <==
\chapter{Generalizations and additional considerations}
\label{cha:generalized-spectral}

So far, we have seen that the spectral method, along with appropriate statistical models, provides a simple yet effective workhorse for statistical estimation. However, the vanilla form of the spectral method, which directly extracts the top eigenspace or singular space of certain data matrices, may not be sufficient. In this chapter, we illustrate modifications to the spectral method, which are often found necessary to further enhance sample efficiency, increase robustness to outliers, incorporate signal priors, and deal with asymmetric perturbations.

%\input{chapters/truncatedWF.tex}

%\input{chapters/truncated_outliers.tex}

%\input{chapters/sparse.tex}

\input{chapters/asymmetric.tex}

\section{Notes}

The first order-wise optimal spectral method  for phase retrieval was proposed by  \citet{chen2015solving}, based on the truncation idea. This method has multiple variants \citep{li2017nonconvex, wang2017solving}, and has been shown to be robust against noise. The precise asymptotic characterization of the spectral method was first obtained in \citet{lu2020phase}, where its sensitivity to model mismatch is studied in \citet{monardo2019sensitivity}. Based on this characterization, \citep{mondelli2017fundamental,luo2019optimal} later devised optimal designs of spectral methods in phase retrieval when the sensing matrix follows the Gaussian design. \cite{ma2019spectral,dudeja2020analysis} considered similar questions when the sensing matrix
is Haar distributed (e.g. an isotropically random unitary matrix).

\citep{fannjiang2020numerics} provided an extensive discussion on initialization strategies for algorithmic phase retrieval, including but not limited to various forms of the spectral method.

Sparse phase retrieval \citep{jagatap2019sample} 

sparse phase retrieval \citep{ma2019spectral}
 
\cite{yuan2013truncated}

sparse spectral method for blind calibration \cite{li2018blind}

Lee and Wu \cite{lee2017near}


 ranking from pairwise comparisons \citep{negahban2016rank,chen2015spectral,chen2017spectral}, 

sparse PCA \cite{amini2008high,JohLu09}

==> chapters/old_notes/old_preliminary.tex <==
\section{Appendix B: Basics of matrix analysis} \label{subsec:Matrix-analysis}

In this section, we review some basic facts in matrix analysis that are useful for the development in Chapter~\ref{{cha:matrix-perturbation}}. 
 

\subsection{Eigenvalues and eigenvectors}

We start with the definition of eigenvalues and eigenvectors of a real
square matrix.

\begin{definition}[Eigenpair]\label{def:eigenpair} Fix a square
matrix $\bm{A}\in\mathbb{R}^{n\times n}$. We say $(\lambda,\bm{v})\in\mathbb{C}\times\mathbb{C}^{n}$
is an \emph{eigenpair} of $\bm{A}$ if $\bm{v}$ is nonzero and 
\begin{equation}
\bm{A}\bm{v}=\lambda\bm{v}.\label{eq:def-eigenpair}
\end{equation}
In particular, the scalar $\lambda$ is an eigenvalue of $\bm{A}$
and $\bm{v}$ is the associated eigenvector. \end{definition}

In words, an eigenvector $\bm{v}$ of $\bm{A}$ does not change its
direction when multiplied by $\bm{A}$ and the eigenvalue $\lambda$
measures the amount of expansion or shrinkage in this linear transformation.
Several remarks regarding Definition~\ref{def:eigenpair} are in
order.
\begin{itemize}
\item The eigenpair (i.e.~the eigenvalue and the associated eigenvector) is only defined
for square matrices. This is implicitly assumed in the definition
of the eigenpair (see~(\ref{def:eigenpair})).
\item Every $n\times n$ square matrix has exactly $n$ (complex) eigenvalues,
possibly with repetitions. To see this, one can transform (\ref{def:eigenpair})
into the identity
\[
\left(\lambda\bm{I}_{n}-\bm{A}\right)\bm{v}=\bm{0}.
\]
Consequently, the scalar $\lambda$ is an eigenvalue of $\bm{A}$
if and only if 
\[
\mathsf{det}\left(\lambda\bm{I}_{n}-\bm{A}\right)=0,
\]
where $\mathsf{det}(\cdot)$ is the determinant of a matrix. Notice that the above relation specifies a polynomial equation of
degree $n$, which by the fundamental theorem of algebra, has exactly
$n$ roots in the complex field (and hence $n$ complex eigenvalues
of~$\bm{A}$).
\item A real matrix can have complex eigenvalues and
complex eigenvectors. Take for instance the matrix
\[
\bm{A}=\left[\begin{array}{cc}
3 & -2\\
4 & -1
\end{array}\right],
\]
where $1+2i$ and $1-2i$ are its two complex eigenvalues. Here $i$
denotes the imaginary unit.
\end{itemize}
With the last remark being said, there exists one important set of
real matrices --- \emph{real symmetric matrices} --- of which the eigenvalues
must be real. This claim is formalized in the following theorem.  

\begin{theorem}[Spectral theorem]\label{thm:spectral} Let $\bm{A}\in\mathbb{R}^{n\times n}$
be a real symmetric matrix. Then there exists $n$ real eigenvalues
$\lambda_{1},\cdots\lambda_{n}\in\mathbb{R}$ and an orthonormal basis
$\bm{u}_{1},\cdots\bm{u}_{n}\in\mathbb{R}^{n}$ such that $\bm{A}\bm{u}_{i}=\lambda_{i}\bm{u}_{i}$.
Equivalently, a real symmetric matrix $\bm{A}$ enjoys the following
spectral decomposition 
\begin{equation}
\bm{A}=\sum_{i=1}^{n}\lambda_{i}\bm{u}_{i}\bm{u}_{i}^{\top}.\label{eq:spectral-decomposition-summation-form}
\end{equation}
%where $\{\lambda_{i}\}_{1\leq i\leq n}$ are the real eigenvalues of $\bm{A}$ and $\{\bm{u}_{i}\}_{1\leq i\leq n}$ is an orthonormal basis of~$\mathbb{R}^{n}$.

\end{theorem}

Since the eigenvalues of real symmetric matrices are guaranteed to
be real numbers, we can therefore order them. From now on, denote
by $\lambda_{i}(\bm{A})$ the $i$th largest eigenvalue of a real
symmetric matrix $\bm{A}\in\mathbb{R}^{n\times n}$. In addition,
we define 
$$\lambda_{\max}(\bm{A})\coloneqq\lambda_{1}(\bm{A}) \quad \mbox{and}
\quad \lambda_{\min}(\bm{A})\coloneqq\lambda_{n}(\bm{A}). $$

To make the formula (\ref{eq:spectral-decomposition-summation-form})
more compact, we denote 
\[
\bm{U}=\left[\begin{array}{ccc}
\rvert &  & \rvert\\
\bm{u}_{1} & \cdots & \bm{u}_{n}\\
\rvert &  & \rvert
\end{array}\right]\in\mathbb{R}^{n\times n},\;\text{and}\;\bm{\Lambda}=\left[\begin{array}{cccc}
\lambda_{1} & 0 & \cdots & 0\\
0 & \lambda_{2} & \cdots & 0\\
\vdots & \vdots & \ddots & \vdots\\
0 & 0 & \cdots & \lambda_{n}
\end{array}\right]\in\mathbb{R}^{n\times n}.
\]
As a result, the decomposition (\ref{eq:spectral-decomposition-summation-form})
can be rewritten as 
\begin{equation}
\bm{A}=\bm{U}\bm{\Lambda}\bm{U}^{\top},\label{eq:spectral-decomposition-multiplication-form}
\end{equation}
in which a real symmetric matrix is decomposed into the multiplications
of orthonormal matrices (i.e.~$\bm{U}$) and a real diagonal matrix
(i.e.~$\bm{\Lambda}$). Another useful way to interpret spectral
decomposition is through the lens of diagonalization. Simple algebraic
manipulation reveals an equivalent form of (\ref{eq:spectral-decomposition-multiplication-form})
\begin{equation}
\bm{U}^{\top}\bm{A}\bm{U}=\bm{\Lambda}.\label{eq:spectral-decomposition-diagonalization-form}
\end{equation}
This essentially tells us that any real symmetric matrix $\bm{A}$
can be \emph{diagonalized }by an orthonormal matrix~(i.e.~$\bm{U}$).

\subsection{Singular values and singular vectors}

As we have pointed out in the remarks following Definition~\ref{def:eigenpair},
a rectangular matrix does \emph{not} have well-defined eigenvalues
and eigenvectors. It is then natural to ask whether there is a similar
decomposition of a general matrix to that of a real symmetric matrix
(cf.~(\ref{eq:spectral-decomposition-multiplication-form})). Fortunately,
a general matrix admits another useful representation: singular value
decomposition (SVD).

\begin{definition}[Singular value decomposition]\label{def:SVD}Let
$\bm{A}\in\mathbb{R}^{m\times n}$ be a general matrix. Without loss
of generality, assume that $m\leq n$. There exists a pair of orthonormal
matrices $\bm{U}\in\mathbb{R}^{m\times m}$ and $\bm{V}\in\mathbb{R}^{n\times n}$
such that 
\begin{equation}\label{eq:SVD}
\bm{A}=\bm{U}\bm{\Sigma}\bm{V}^{\top},
\end{equation}
where $\bm{\Sigma}$ is a rectangular diagonal matrix with 
\[
\bm{\Sigma}=\left[\begin{array}{cccccc}
\sigma_{1} & 0 & \cdots & \cdots & 0 & 0\\
0 & \sigma_{2} & \cdots & \cdots & 0 & 0\\
\vdots & \vdots & \ddots & \vdots & \vdots & \vdots\\
0 & 0 & \cdots & \sigma_{m} & 0 & 0
\end{array}\right]\in\mathbb{R}^{m\times n}
\]
and $\sigma_{1}\geq\sigma_{2}\geq\cdots\geq\sigma_{m}\geq0$. The
decomposition (\ref{eq:SVD}) is called singular value decomposition,
where the nonnegative real numbers $\{\sigma_{i}\}_{1\leq i\leq n}$
are the singular values of $\bm{A}$ and the columns in $\bm{U}$
(resp.~$\bm{V}$) are the left (resp.~right) singular vectors of
$\bm{A}$. \end{definition}

Similar to the eigenvalues of real symmetric matrices, the singular
values of a general matrix are guaranteed to be real. \yc{a bit redundant since the above already said all singular values are above zero (hence must be real).}As a result,
for any $1\leq i\leq\min\{m,n\}$, we define $\sigma_{i}(\bm{A})$
to be $i$th largest singular value of $\bm{A}$, define $\sigma_{\max}(\bm{A})\coloneqq\sigma_{1}(\bm{A})$
(resp.~$\sigma_{\min}(\bm{A})\coloneqq\sigma_{\min\{m,n\}}(\bm{A})$)
to be the largest (resp.~smallest) singular values of $\bm{A}$.

It is straightforward to read the rank of a matrix from its singular
values in that the rank is equal to the number of nonzero singular
values. If the rank $r$ of a matrix $\bm{A}\in\mathbb{R}^{m\times n}$
is smaller than $\min\{m,n\}$, it is often more economical to represent
the matrix using the \emph{compact SVD }
\begin{equation}
\bm{A}=\bm{U}_{r}\bm{\Sigma}_{r}\bm{V}_{r}^{\top},\label{eq:compact-SVD}
\end{equation}
where $\bm{U}_{r}$ (resp.~$\bm{V}_{r}$) is the first $r$ columns
of $\bm{U}$ (resp.~$\bm{V}$) and $\bm{\Sigma}_{r}$ is the upper
left block of $\bm{\Sigma}$ with size $r$.

Having introduced two decompositions, it is instrumental to compare
the singular value decomposition of a general matrix (cf.~Definition~\ref{def:SVD})
with the spectral decomposition of a real symmetric matrix (cf.~Theorem~(\ref{thm:spectral})).
First, the eigenvalues of a real symmetric matrix are not necessarily
nonnegative whereas singular values must be. Second, as claimed in
(\ref{eq:spectral-decomposition-diagonalization-form}), any real
symmetric matrix can be diagonalized by a single orthonormal matrix.
However, this may not hold true for a general matrix, nevertheless,
SVD points out a way to diagonalize a matrix using two orthonormal
matrices. To see this, one can equate (\ref{eq:SVD}) with

\[
\bm{U}^{\top}\bm{A}\bm{V}=\bm{\Sigma}.
\]
Last but not least, singular value decomposition and spectral decomposition
are inherently related. It is an easy exercise to see that the columns
of $\bm{U}$ (resp.~$\bm{V}$) are eigenvectors of $\bm{A}\bm{A}^{\top}$
(resp.~$\bm{A}^{\top}\bm{A}$). In addition, the singular values
of $\bm{A}$ are nonnegative square roots of the eigenvalues of either
$\bm{A}\bm{A}^{\top}$ or $\bm{A}^{\top}\bm{A}$ (modulo zero singular
values). This connection shall prove useful in later discussions.

\subsection{Matrix norms}

To measure the size of the perturbation (e.g.~$\bm{E}$), we need
to introduce appropriate metrics~/~norms on the space of matrices.
Among all matrix norms, unitarily invariant norms are of most interest
to us. \begin{definition}[Unitarily invariant norms]A matrix norm
$\vertiii{\cdot}$ on $\mathbb{R}^{m\times n}$ is unitarily invariant
if
\[
\vertiii{\bm{A}}=\vertiiibig{\bm{U}^{\top}\bm{A}\bm{V}}
\]
for any matrix $\bm{A}\in\mathbb{R}^{m\times n}$ and any two orthogonal
matrices $\bm{U}\in\mathbb{R}^{m\times m}$ and $\bm{V}\in\mathbb{R}^{n\times n}$.
\end{definition}

Two prominent examples include the Frobenius norm and the operator
norm

\begin{equation}
\left\Vert \bm{A}\right\Vert _{\mathrm{F}}=\sqrt{\sum_{i,j}A_{ij}^{2}}\qquad\text{and}\qquad\left\Vert \bm{A}\right\Vert =\max_{\bm{x}\in\mathbb{R}^{n}:\bm{x}\neq\bm{0}}\frac{\left\Vert \bm{A}\bm{x}\right\Vert _{2}}{\left\Vert \bm{x}\right\Vert _{2}}.\label{eq:def-fro-op-norm}
\end{equation}
To see why both $\|\cdot\|_{\mathrm{F}}$ and $\|\cdot\|$ are unitarily
invariant norms, we have the following important characterizations
\[
\left\Vert \bm{A}\right\Vert _{\mathrm{F}}=\sqrt{\sum_{i=1}^{\min\{m,n\}}\sigma_{i}^{2}\left(\bm{A}\right)}\qquad\text{and}\qquad\left\Vert \bm{A}\right\Vert _{\mathsf{2}}=\sigma_{1}\left(\bm{A}\right),
\]
where we recall that $\sigma_{1}(\bm{A})\geq\sigma_{2}(\bm{A})\geq\cdots\geq\sigma_{\min\{m,n\}}(\bm{A})\geq0$
are the singular values of $\bm{A}$ in descending order.

Last but not least, unitarily invariant norms enjoy the following
nice properties.

\begin{proposition}\label{prop:unitary_norm_relation}Let $\vertiii{\cdot}$ be any unitarily invariant norm.
One has 
\begin{align*}
\vertiii{\bm{A}\bm{B}} & \leq\vertiii{\bm{A}}\left\Vert \bm{B}\right\Vert _{2}, &  & \vertiii{\bm{A}\bm{B}}\leq\vertiii{\bm{B}}\left\Vert \bm{A}\right\Vert _{2},\\
\vertiii{\bm{A}\bm{B}} & \geq\vertiii{\bm{A}}\sigma_{\min}\left(\bm{B}\right), &  & \vertiii{\bm{A}\bm{B}}\geq\vertiii{\bm{B}}\sigma_{\min}\left(\bm{A}\right).
\end{align*}
\end{proposition}
\begin{proof}See Theorem 3.9 in \citep{stewart1990matrix}.\end{proof}

\subsection{Perturbation bounds for eigenvalues and singular values}


In this section, we review classical perturbation
bounds for eigenvalues of symmetric matrices and singular values for general matrices. 

\begin{lemma}[Weyls's inequality]\label{lemma:weyl}Let
$\bm{A},\bm{E}\in\mathbb{R}^{n\times n}$ be two real symmetric matrices.
For every $1\leq i\leq n$, we have 
\begin{equation}
\left|\lambda_{i}\left(\bm{A}\right)-\lambda_{i}\left(\bm{A} +\bm{E}\right)\right|\leq\left\Vert \bm{E}\right\Vert .\label{eq:weyl}
\end{equation}
\end{lemma}
\begin{proof}See Equation (1.63) in \citep{Tao2012RMT}. \end{proof}


An immediate implication of Lemma~\ref{lemma:weyl} is that the eigenvalues
of a real symmetric matrix are stable against perturbations. Similar bounds hold for singular values.


\begin{lemma}[Wely's inequality for singular values]\label{lemma:weyls-singular-value}Let
$\bm{A},\bm{E}\in\mathbb{R}^{m\times n}$ be two general matrices.
Without loss of generality, assume that $m\leq n$. Then for every
$1\leq i\leq m$, one has 
\[
\left|\sigma_{i}\left(\bm{A}+\bm{E}\right)-\sigma_{i}\left(\bm{A}\right)\right|\leq\left\Vert \bm{E}\right\Vert .
\]
\end{lemma}
\begin{proof}See Exercise 1.3.22 in \citep{Tao2012RMT}. \end{proof}
Again, Lemma~\ref{lemma:weyls-singular-value} reveals that singular
values are \emph{stable }with respect to small perturbations.


%\chapter{Random matrix theory}
%
%\cm{Need to motivate why we need these. }
%
%As we have mentioned in Section~XXX, we often observe
%
%One quantitative version of the central limit theorem \cm{TODO}
%
%
%\begin{theorem}[Bernstein's inequality]Let $\{x_{i}\}_{1\leq i\leq n}$
%be a sequence of independent random variables. Suppose that for each
%$1\leq i\leq n$, $\mathbb{E}[x_{i}]=0$ and $|x_{i}|\leq B$ almost
%surely. Then we have for all $t\geq0$ 
%\[
%\mathbb{P}\left(\left|\sum_{i=1}^{n}x_{i}\right|\geq t\right)\leq2\exp\left(\frac{-t^{2}/2}{V+Bt/3}\right),
%\]
%where $V$ is the variance statistic 
%\[
%V\coloneqq\left|\sum_{i=1}^{n}\mathbb{E}\left[x_{i}^{2}\right]\right|.
%\]
%\end{theorem}




==> chapters/old_notes/sparse.tex <==

\section{Truncated spectral method for sparse phase retrieval}\label{sec:spectral_init_spr}

Next, we briefly discuss how the spectral method can be modified to incorporate structural priors. In many problems of practical interest, we might be given some prior knowledge about the signal of interest, encoded by a constraint set $\bm{x}_{\star}\in\mathcal{C}\subset \mathbb{R}^n$. Therefore, it is natural to apply projection to enforce the desired structural constraints. A special structure that will receive special attention is the sparsity prior, where it is known {\em a priori} that the signal of interest $\bm{x}_{\star} $ is $k$-sparse, where $k\ll n$. We shall illustrate this idea through the application of sparse phase retrieval.


\paragraph{Sparse phase retrieval.} Consider the phase retrieval problem formulated in Section~\ref{sec:formulation-PR}, where we now additionally assume $\bx_{\star}$ is  $k$-sparse, i.e. $\| \bx_{\star}\|_0 = k$.  The sparse phase retrieval problem has numerous applications in computational imaging \citep{soltanolkotabi2017structured,shechtman2014gespar,chen2015exact}, as it offers the premise to further reducing the sampling cost by exploiting the sparsity structure.
A simple idea is to first identify the support of $\bx_{\star}$, and then try to estimate  the nonzero values by applying the spectral method over the submatrix of $\bM$ on the estimated support. Towards this end, we recall that 
$$\mathbb{E}[\bM] = 2\bx_{\star}\bx_{\star}^{\top}+ \|\bx_{\star}\|_2^2\bI_n, $$ 
and therefore the larger ones of the diagonal entries of $\bM$ are more likely to be in the support of $\bx_{\star}$. In light of this, a simple thresholding strategy adopted in \cite{cai2016optimal} is to compare $M_{i,i}$ against some preset threshold $\gamma$:
$$ \hat{\mathcal{S}} = \{i: \; Y_{i,i}> \gamma \} .$$
The nonzero part of $\bx_{\star}$ is then found by applying the spectral method outlined in Section~\ref{sec:phase_retrieval} to 
$$\bm{M}_{\hat{\mathcal{S}}} =\frac{1}{m}\sum_{i=1}^m y_i \bm{a}_{i,\hat{\mathcal{S}}}\bm{a}_{i,\hat{\mathcal{S}}}^{\top}, $$ 
where $\bm{a}_{i,\hat{\mathcal{S}}}$ is the subvector of $\bm{a}_{i}$ coming from the support $\hat{\mathcal{S}}$. 
In short, this strategy provably leads to a reasonably good initial estimate, as long as the sample size $m \gtrsim k^2 \log m$ is sufficiently large; the exact form of the theory can be found in \cite{cai2016optimal}. 
See also \citep{wang66sparse} for a more involved approach, which provides better empirical performance.
 
 
\begin{remark}
Careful readers might realize that the sample complexity of the sparse spectral method is much larger than the information-theoretical lower bound established in, e.g., \cite{eldar2014phase}. 
Unfortunately, to date there is no tractable  procedure that can provably guarantee a consistent estimate of $\bm{x}_\star$ when $m = O( k\log n) $. Rather, all known computationally feasible algorithms (both convex and nonconvex)  require a sample complexity at least on the order of $k^2 \log n$ under the Gaussian design (i.e. Assumption~\ref{assump:pr-gaussian}), unless $k$ is sufficiently large or other structural information is available \citep{li2013sparse,oymak2012simultaneously,chen2015exact,cai2016optimal,jagatap2017fast}.  All in all, there seems to exist a computational barrier for sparse phase retrieval between the sample complexity requirements for computationally efficient procedures and the information-theoretic limit. 
\end{remark}

 

==> chapters/old_notes/truncatedWF.tex <==

\section{Truncated spectral method for sample efficiency} \label{sec:improved-spectral-truncated}

The generic recipe for spectral methods described in the previous chapters works well when one has  sufficient samples compared to the underlying signal dimension. It might not be effective though if the sample complexity is on the order of  the information-theoretic limit. 

In what follows, we use phase retrieval, discussed in Section~\ref{sec:phase_retrieval}, to demonstrate the underlying issues and how to address them\footnote{Strategies of similar spirit have been proposed for other problems; see, e.g.,~\citep{keshavan2010matrix} for matrix completion. }. Recall that Theorem~\ref{thm:PR-L2-performance} requires a sample complexity $m \gtrsim n  \log^3 n$, which is a few logarithmic factor larger than the  signal dimension $n$.  
%For matrix completion, we assume the sampling probability $p > \log^3 n/ n$ in Theorem~\ref{thm:spectral_MC}.
%
What happens if we only have access to $m \asymp n$ samples, which is the information-theoretic limit (order-wise) for phase retrieval? In this more challenging regime, it turns out that we have to modify the standard recipe by applying appropriate preprocessing before forming the surrogate matrix $\bm{M}$ in \eqref{eq:D_PR_org}.


We start by explaining why the surrogate matrix $\bm{M}$ in \eqref{eq:D_PR_org} for phase retrieval must be suboptimal in terms of sample complexity. For all $1 \le j \le m$,
\begin{equation*}
	\norm{\bm{M}} \ge \frac{\va_j^\top \bm{M} \va_j}{\va_j^\top \va_j}=  \frac{1}{m} \sum_{i=1}^m y_i \frac{(\va_i^\top \va_j)^2}{\va_j^\top \va_j} \geq \frac{1}{m}  y_j  \| \va_j \|_2^2.
\end{equation*}
%
In particular, taking $j = i^\ast  = \underset{{1 \le i \le m}}{\arg \max} \ y_i$ gives us
\begin{equation}\label{eq:bound_id2}
	\norm{\bm{M}} \ge \frac{(\max_i y_i) \| \va_{i^\ast} \|_2^2}{m}.
\end{equation}
Under the Gaussian design, $\set{y_i / \| \vxp \|_2^2}$ is a collection of i.i.d.~$\chi^2$ random variables with 1 degree of freedom. It follows from well-known estimates in extreme value theory \citep{Ferguson:1996} that 
\[
\max_{1\le i \le m} \, y_i \approx 2\|\vxp\|_2^2 \log m,\qquad \text{as}\; m \to \infty.
\] 
Meanwhile, note that $\| \va_{i^\ast} \|_2^2  \approx n$ for $n$ sufficiently large. It follows from \eqref{eq:bound_id2} that
\begin{equation}\label{eq:PR_sc}
	\norm{\bm{M}} \ge \big(1+o(1)\big)  \frac{ n \log m}{  m} \|\vxp\|_2^2  .
\end{equation}
%

%These estimates can be made precise as follows.
%\begin{lemma}\label{lemma:T_id}
%Suppose the sensing vectors $\set{\va_i}$ are drawn from the i.i.d. Gaussian distribution. Then
%\[
%\norm{\mD - \mathbb{E}[\mD]} > \norm{\vxp}^2 (n \log m) / m - 2 \norm{\vxp}^2  - 1
%\]
%with probability at least $1 - \mathcal{O}(1/n^2)$.
%\end{lemma}

%Recall that $\mathbb{E}[\bm{Y}] = \vxp \vxp^\top + \| \vxp\|_2^2 \boldsymbol{I}_n$.  Its spectral norm is bounded and its leading eigenvector is exactly the true object $\vxp$. Our goal is to make sure the noisy matrix $\bm{Y}$ is close to $\EE[\bm{Y}]$ so that the principal eigenvector of $\bm{Y}$ stays close to that of $\EE[\bm{Y}]$. 
% = \vxp \vxp^\top + \| \vxp\|_2^2 \boldsymbol{I}_n

Recall that $\mathbb{E}[\bm{M}] = 2 \vxp \vxp^\top +  \| \vxp\|_2^2 \boldsymbol{I}_n$ has a bounded spectral norm, then \eqref{eq:PR_sc} implies that, to keep the deviation between $\bm{M}$ and $\mathbb{E}[\bm{M}]$ well-controlled, we must at least have
\[
\frac{n \log m}{ m} \lesssim 1.
\]
This condition, however, cannot be satisfied when we have linear sample complexity $m \asymp  n$. This explains why we need a sample complexity $m \gg n \log n$ in Theorem~\ref{thm:PR-L2-performance}. 
%Indeed, in \cite{netrapalli2013phaseAM}, the authors established performance guarantees for the spectral method by assuming $m =  c \cdot n \log^3 n$ (for some sufficiently large $c$), and this requirement was later reduced to $m = c \cdot n \log n$ in \cite{candes2015phase}. 

The above diagnosis also suggests an easy fix: since the main culprit lies in the fact that $\max_i y_i$ is unbounded (as $m \to \infty$), we can apply a preprocessing function $\mathcal{T}(\cdot)$ to $y_i$ to keep the quantity bounded. Indeed, this is the key idea behind the {\em truncated spectral method} proposed by \cite{chen2015solving}, in which the surrogate matrix is modified as
%
\begin{equation}
	\label{eq:D_PR_T}
	\bm{M}_{\mathcal{T}} := \frac{1}{m} \sum_{i=1}^m \mathcal{T}(y_i) \va_i \va_i^\top,
\end{equation} 
%
where 
\begin{equation}\label{eq:trimming}
\mathcal{T}(y) := y \charfn_{\set{\abs{y} \le  \frac{\gamma}{m} \sum_{i=1}^m y_i}}
\end{equation}
for some predetermined truncation threshold $\gamma$. The initial point $\bm{x}_0$ is then formed by scaling the leading eigenvector of $\bm{M}_{\mathcal{T}}$ to have roughly the same norm of $\bx_{\star}$, which can be estimated by $\overline{y} =\frac{1}{m} \sum_{i=1}^m y_i $. This is essentially performing a trimming operation, removing any entry of $y_i$ that bears too much influence on the leading eigenvector.  The trimming step turns out to be very effective, allowing one to achieve order-wise optimal sample complexity. The following theorem is due to \cite{chen2015solving}. 
%
%\begin{align}
%	\label{eq:init-spectral-proc}
%	\bm{x}_0 = \sqrt{\lambda}\bm{u},
%\end{align}
%
%where $\lambda$ and $\bm{u}$ are the leading eigenvalue and eigenvector of $\bm{Y}_{\mathcal{T}}$, respectively. 


%
\begin{theorem}[$\mathsf{Truncated~spectral~method~for~phase~retrieval}$]
	\label{thm:truncated-PR}
	Consider phase retrieval in Section~\ref{sec:phase_retrieval}. Fix any $\zeta > 0$, and suppose $m \ge c_0 n $ for some sufficiently large constant $c_0>0$.  Then the truncated spectral estimate obeys
\[
	\mathsf{dist}(\bm{x},\bm{x}^{\star})  \le \zeta \| \vxp \|_2
\]
with probability at least $1 - O(n^{-2})$.
\end{theorem}

Subsequently, several different designs of the preprocessing function have been proposed in the literature. One example was given in \cite{wang2017solving}, where
\begin{equation}\label{eq:subset}
	\mathcal{T}(y)  = \charfn_{\set{y \ge \gamma  }},
\end{equation}
%
where $\gamma$ is the $(cm)$-largest value (e.g.~$c=1/6$) in $\{ y_j \}_{1\le j\le m}$. In words, this method only employs a subset of design vectors that are better aligned with the truth $\bm{x}_{\star}$.  By properly tuning the parameter $c$, this truncation scheme performs competitively as the scheme in \eqref{eq:trimming}.

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.8\textwidth]{figures/stanford} \\
(a) ground truth \\
\includegraphics[width=0.8\textwidth]{figures/stanford_quad_init_WF} \\
(b) initialization via the vanilla spectral method \\
\includegraphics[width=0.8\textwidth]{figures/stanford_quad_init_TWF}  \\
(c) initialization via the truncated spectral method
\end{center}
	\caption{Illustration of signal recovery using the vanilla spectral method and the truncated spectral method in phase retrieval. Here, \textbf{add parameter settings}. } \label{fig:phase_retrieval_twf}
\end{figure}



==> chapters/old_notes/truncated_outliers.tex <==

\section{Truncated spectral method for removing sparse outliers}

When the samples are susceptible to adversarial entries, the spectral method might not work properly even with the presence of a single outlier whose magnitude can be arbitrarily large to perturb the leading eigenvector of the data matrix $\bm{M}$. Therefore, the spectral method needs to be modified carefully in order to still function properly in the presence of outliers.

\paragraph{Median-truncated spectral method.} One strategy to remove outliers is to truncate away spurious samples based on the sample median, as the median is known to be robust against arbitrary outliers \citep{zhang2016provable,li2017nonconvex}. We illustrate this median-truncation approach through an example of robust phase retrieval \citep{zhang2016provable}, where we assume a subset of samples in \eqref{eq:PR-samples} is corrupted arbitrarily, with their index set denoted by $\mathcal{S}$ with $|\mathcal{S}|=\alpha  m$, $\alpha \in (0,1/2]$ is the faction of outliers. Mathematically, the measurement  model in the presence of outliers is given by
%
\begin{equation} \label{eq:robust_pr_model}
	y_i = \begin{cases}
(\ba_i^\top\bx_{\star})^2, \quad  & i \notin \mathcal{S}, \\
\mathsf{arbitrary} , & i \in \mathcal{S}. 
	\end{cases}
\end{equation}
%
The goal is to still recover $\bm{x}_{\star}$ in the presence of many outliers (e.g.~a constant fraction of measurements are outliers). To mitigate this issue, a median-truncation scheme was proposed in \cite{zhang2016provable,li2017nonconvex}, where
\begin{equation}\label{eq:T_median}
	\mathcal{T}(y)  = y \charfn_{\set{y_i \leq \gamma \, \mathsf{median}\{ y_j \}_{j=1}^m}}
\end{equation}
for some predetermined constant $\gamma >0$, $\mathsf{median}\{ y_j \}_{j=1}^m $ is the median of the samples $\{ y_j \}_{j=1}^m$. The data matrix $\bM$ is then constructed via \eqref{eq:D_PR_T} using the above preprocessing function.

 By including only a subset of samples whose values are not excessively large compared with the sample median of the samples, the preprocessing function in \eqref{eq:T_median} makes the spectral method more robust against sparse and large outliers.
The following theorem is due to \cite{zhang2016provable}. 
\begin{theorem} 
	\label{thm:truncated-PR-init}
	Consider the robust phase retrieval problem in \eqref{eq:robust_pr_model}, and fix any $\zeta > 0$. There exist some constants  $c_0, c_1>0$ such that if 
$m\geq c_{0}n$ and $\alpha\leq c_1$, then the median-truncated spectral estimate obeys
\[
	\mathsf{dist}(\bm{x},\bm{x}^{\star})  \le \zeta \| \vxp \|_2
\]
with probability at least $1 - O(n^{-2})$.
\end{theorem}

Theorem~\ref{thm:truncated-PR-init} suggests that even with a constant fraction of outliers, the median-truncated spectral method can still robustly estimate $\bm{x}^{\star}$ with a near-optimal number of measurements $m=O(n)$, thus further enhancing the resilience of the truncated spectral method in the presence of adversarial corruptions.

%median-TWF needs O(n) sample for initialization.
\paragraph{Hard-thresholded spectral method.}
The idea of applying truncation to form a spectral estimate is also used in the robust PCA problem \citep{chandrasekaran2011siam,candes2009robustPCA,vaswani2017robust}, when we are provided an upper bound on the fraction of outliers. 
Suppose we are given a matrix $\bm{\Gamma}_{\star}\in\mathbb{R}^{n_1\times n_2}$ that is a superposition of a rank-$r$ matrix $\bm{M}_{\star}\in\mathbb{R}^{n_1\times n_2}$ and a sparse matrix $\bm{S}_{\star}\in\mathbb{R}^{n_1\times n_2}$:
%
\begin{equation}\label{eq:rpca_decomp}
\bm{\Gamma}_{\star} = \bm{M}_{\star} + \bm{S}_{\star}.
\end{equation}
%
The goal is to separate $\bm{M}_{\star}$ and $\bm{S}_{\star}$ from the (possibly partial) entries of $\bm{\Gamma}_{\star}$. This problem is also known as {\em robust PCA}, since we can think of it as recovering the low-rank factors of  $\bm{M}_{\star}$ when the observed entries are corrupted by {\em sparse outliers} (modeled by $\bm{S}_{\star}$). The problem spans numerous applications in computer vision, medical imaging, and video surveillance. 

Similar to the matrix completion problem, we assume the random sampling model \eqref{assump:mc-bernoulli}, where $\Omega$ is the set of observed entries. 
In order to make the problem well-posed, we need the incoherence parameter of $\bM_{\star}$ as defined in Definition~\ref{assump:mc-incoherence} as well, which precludes $\bM_{\star}$ from being too spiky.  In addition, it is sometimes convenient to introduce the following deterministic condition on the sparsity pattern and sparsity level of $\bm{S}_{\star}$,  originally proposed by \cite{chandrasekaran2011siam}. Specifically, it is assumed that the non-zero entries of $\bm{S}_{\star}$ are ``spread out'', where there are at most a  fraction $\alpha$ of non-zeros per row\,/\,column. Mathematically, this means:

\begin{assumption}
	It is assumed that $\bS_{\star}\in\mathcal{S}_\alpha\subseteq \mathbb{R}^{n_1\times n_2}$, where
%
\begin{equation}
	\mathcal{S}_\alpha := \left\{\bS \,:\,  \|(\bS_{\star})_{i,\cdot}\|_0 \leq \alpha n_2, \; \|(\bS_{\star})_{\cdot,j}\|_0 \leq \alpha n_1, \forall i,j \right\}. 
\end{equation}
%
\end{assumption}


Since the observations are also potentially corrupted by large but sparse outliers, it is useful to first clean up the observations $(\bm{\Gamma}_{\star})_{i,j} = (\bm{M}_{\star})_{i,j} + (\bm{S}_{\star})_{i,j}$ before constructing the matrix $\bM$ as in \eqref{eq:rescaled-M-matrix-completion-l2}. Indeed, this is the strategy proposed in \cite{yi2016fast}. 
%For simplicity, we present in what follows only the results for the fully observed case. 
To proceed, we start by forming an estimate of the sparse outliers via the hard-thresholding operation as
\begin{equation}\label{eq:hard_threshodling_init}
\bm{S}_{0}=\mathcal{H}_{c\alpha np}\big(\mathcal{P}_{\Omega}(\bm{\Gamma}_{\star} )\big).
\end{equation}
%We start by forming an estimate of the sparse outliers. Let
%\[
%\mathcal{T}_{\alpha}[\bm{\Gamma}] = \begin{cases}
%\bm{\Gamma}_{i,j}, &\text{if } \abs{\bm{\Gamma}_{i,j}} \ge \abs{\bm{\Gamma}_{(i, \cdot)}^{(\alpha n_2)}} \text{ and } \abs{\bm{\Gamma}_{i,j}} \ge \abs{\bm{\Gamma}_{(\cdot, j)}^{(\alpha n_1)}} \\
%0,&\text{otherwise}
%\end{cases},
%\]
%where $\bm{\Gamma}_{(i, \cdot)}^{(k)}$ (resp. $\bm{\Gamma}_{(\cdot, j)}^{(\alpha n_1)}$) denotes the $k$th largest entry of $\bm{\Gamma}_{(i, \cdot)}$ (resp. $\bm{\Gamma}_{(\cdot, j)}$). 
where $c>0$ is some predetermined constant (e.g.~$c=3$) and $\mathcal{P}_{\Omega}$ is defined in \eqref{defn:Pomega}. Here, $\mathcal{H}_l(\cdot)$ is the hard-thresholding operator defined as
%
\[
	[\mathcal{H}_{l}(\bA)]_{j,k} := \begin{cases}  A_{j,k},  &\text{if }|A_{j,k}|\geq |A_{j,\cdot}^{(l)}| \text{ and }
							|A_{j,k}|\geq |A_{\cdot,k}^{(l)}|,  \\
							0, & \text{otherwise,}
					  \end{cases}
\]
where 
$A_{j,\cdot}^{(l)}$ (resp.~$A_{\cdot,k}^{(l)}$) denotes the $l$th largest entry (in magnitude) in the $j$th row (resp.~column) of $\bm{A}$.
The  idea is simple: an entry is likely to be an outlier if it is simultaneously among the largest entries in the corresponding row and column. Armed with this estimate, we form the matrix $\bM$ as
%
\begin{equation}
	\label{eq:Y-RPCA}
	\bm{M} =\frac{1}{p} \mathcal{P}_{\Omega}(\bm{\Gamma}_{\star}   - \bm{S}_{0}).
\end{equation}

 
%	


One can then apply the spectral method to $\bm{M}$ in \eqref{eq:Y-RPCA} (similar to the matrix completion case). This approach enjoys the following performance guarantee, due to \cite{yi2016fast}; see also \citep{cherapanamjeri2017nearly}.
%
\begin{theorem} \label{thm:spectral_RPCA}
Suppose that the robust PCA problem. If the sample size and the sparsity fraction satisfy $n_1  p\geq c_0  \kappa^2 \mu r  \log n_2$ and $\alpha\leq c_1/( \mu \kappa  r )$ for
	some sufficiently large (resp. small) constant $c_0>0$ (resp. $c_1>0$), then 
with probability at least $1-O\left(n^{-1}\right)$,  
%
	\[
  \max\Big\{ \mathsf{dist}\left(\bm{U},\bm{U}^{\star}\right),\mathsf{dist}\left(\bm{V},\bm{V}^{\star}\right) \Big\}  \leq  c_2 \alpha \mu r \kappa + c_3 \kappa \sqrt{\frac{\mu r \log n_2}{n_1 p}},
	\]	
for some constants $c_2, c_3>0$.
\end{theorem}

It can be seen that Theorem~\ref{thm:spectral_RPCA} reduces to Theorem~\ref{thm:mc-l2-subspace} for the case of matrix completion when there are no outliers, i.e. $\alpha =0$. Therefore, the truncated spectral method injects additional robustness properties to the spectral method without hurting its performance in the outlier-free case, hence it is resilient in an oblivious fashion.   




==> journaldata/ACC-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

%\journalchiefeditor{Stefan J. Reichelstein}{Stanford University\\United States}



\subsection{Executive Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Robert Bushman}{The University of North Carolina at Chapel Hill}
\journaleditor{Sunil Dutta}{University of California at Berkeley}
\journaleditor{Stephen Penman}{Columbia University}
\journaleditor{Stefan J. Reichelstein, Managing editor}{Stanford University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACC-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{ACCcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {ACCcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Accounting}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACC}
\journalurl        {http://www.nowpublishers.com/ACC}
\journalissnprint  {1554-0642}
\journalissnonline {1554-0650}
\journaldoi        {10.1561/14}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Auditing}
\item{Corporate Governance}
\item{Cost Management}
\item{Disclosure}
\item{Event Studies/Market Efficiency Studies}
\item{Executive Compensation}
\item{Financial Reporting}
\item{Management Control}
\item{Performance Measurement}
\item{Taxation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{The Role of Stakeholders in Corporate Governance: A View from\\ Accounting Research}\\
Gaizka Ormazabal
\\ISBN: 978-1-68083-396-6
\\
\\
\noindent \textit{Financial Analysts and Their Contribution to Well-Functioning Capital Markets}\\
Mark Bradshaw, Yonca Ertimur and Patricia O'Brien
\\ISBN: 978-1-68083-354-6
\\
\\
\noindent \textit{Rethinking Financial Reporting: Standards, Norms and Institutions}\\
Shyam Sunder
\\ISBN: 978-1-68083-144-3


==> journaldata/ACG-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Douglas Cumming}{Florida Atlantic University\\USA}
\journalchiefeditor{Geoffrey Wood}{Western University\\Canada}



\subsection{Associate Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Renee Adams}{University of Oxford}
\journaleditor{Lucian Bebchuk}{Harvard University}
\journaleditor{William Judge}{Old Dominion University}
\journaleditor{Mark Roe}{Harvard University}
\journaleditor{Rene Stulz}{Ohio State University}
\journaleditor{James Westphal}{University of Michigan}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACG-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ACGcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ACGcolor} %a color name. 
\journaltitle      {Annals of Corporate Governance}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACG}
\journalurl        {http://www.nowpublishers.com/ACG}
\journalissnprint  {2381-6724}
\journalissnonline {2381-6732}
\journaldoi        {10.1561/109	}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
Annals of Corporate Governancepublishes
 articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Boards of Directors}
\item{Ownership}
\item{National Corporate Governance Mechanisms}
\item{Comparative Corporate Governance Systems}
\item{Self Governance}
\item{Teaching Corporate Governance}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
 Annals of Corporate Governance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Leveraged Buyouts: Motives and Sources of Value}\\
Luc Renneboog and Cara Vansteenkiste
\\ISBN: 978-1-68083-274-7
\\
\\
\noindent \textit{Microfinance: What Do We Know? Where Do We Go?}\\
Sugato Chakravarty and Mariya Pylypiv
\\ISBN: 978-1-68083-270-9
\\
\\
\noindent \textit{Board Involvement in the Strategic Decision Making Process:\\ A Comprehensive Review}\\
William Q. Judge and Till Talaulicar
\\ISBN: 978-1-68083-260-0
\\
\\
\noindent \textit{Understanding Boards of Directors: A Systems Perspective}\\
Jay W. Lorsch
\\ISBN: 978-1-68083-246-4


==> journaldata/ASTP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ASTP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ASTP-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Policies for the Provision of Finance to Science-based Entrepreneurship}\\
Alice Civera, Michele Meoli and Silvio Vismara\\
ISBN: 978-1-68083-352-2\\
\\
\noindent \textit{The Roles and Impacts of Technical Standards on Economic Growth and Implications for Innovation Policy}\\
Gregory Tassey\\
ISBN: 978-1-68083-316-4\\
\\
\noindent \textit{Bureaucratization in Academic Research Policy: What Causes It?}\\
Barry Bozeman and Jiwon Jung\\
ISBN: 978-1-68083-262-4\\
\\
\noindent \textit{Advanced Manufacturing: A New Policy Challenge}\\
William B. Bonvillian\\
ISBN: 978-1-68083-240-2

==> journaldata/CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Brian Curless}{University of Washington}
\journalchiefeditor{William T. Freeman}{MIT}
\journalchiefeditor{Luc Van Gool}{KU Leuven and ETH Zurich}
%\end{multicols*}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Microsoft Research}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
%\columnbreak
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Aaron Hertzmann}{Adobe Research}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Georgia Tech}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{James O'Brien}{Berkeley}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
%\columnbreak
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {CGVcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\
\\
\noindent \textit{The Path to Path-Traced Movies}\\
Per H. Christensen and Wojciech Jarosz\\
ISBN: 978-1-68083-210-5\\
\\
\noindent \textit{(Hyper)-Graphs Inference through Convex Relaxations and Move Making Algorithms}\\
Nikos Komodakis, M. Pawan Kumar and Nikos Paragios\\
ISBN: 978-1-68083-138-2\\
\\
\noindent \textit{A Survey of Photometric Stereo Techniques}\\
Jens Ackermann and Michael Goesele\\
ISBN: 978-1-68083-078-1\\
\\
\noindent \textit{Multi-View Stereo: A Tutorial}\\
Yasutaka Furukawa and Carlos Hernandez\\
ISBN: 978-1-60198-836-2

==> journaldata/CIT-editorialboard.tex <==
\begin{editorialboard}

%\subsection{Editor-in-Chief}

%\journalchiefeditor{Helmut B\"{o}lcskei}{ETH Zurich\\Switzerland}



\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Venkat Anantharam}{UC Berkeley}
\journaleditor{Giuseppe Caire}{TU Berlin}
\journaleditor{Daniel Costello}{University of Notre Dame}
\journaleditor{Anthony Ephremides}{University of Maryland}
%\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Albert Guillen i Fabregas}{Pompeu Fabra University}
\journaleditor{Dongning Guo}{Northwestern University}
\journaleditor{Dave Forney}{MIT}
\journaleditor{Te Sun Han}{University of Tokyo}
\journaleditor{Babak Hassibi}{Caltech}
\journaleditor{Michael Honig}{Northwestern University}
%\journaleditor{Tara Javidi}{UC San Diego}
%\columnbreak
\journaleditor{Ioannis Kontoyiannis}{Cambridge University}
\journaleditor{Gerhard Kramer}{TU Munich}
\journaleditor{Amos Lapidoth}{ETH Zurich}
\journaleditor{Muriel Medard}{MIT}
\journaleditor{Neri Merhav}{Technion}
\journaleditor{David Neuhoff}{University of Michigan}
\journaleditor{Alon Orlitsky}{UC San Diego}
\journaleditor{Yury Polyanskiy}{MIT}
\journaleditor{Vincent Poor}{Princeton University}
%\journaleditor{Maxim Raginsky}{UIUC}
\journaleditor{Kannan Ramchandran}{UC Berkeley}
\journaleditor{Igal Sason}{Technion}
%\columnbreak
\journaleditor{Shlomo Shamai}{Technion}
\journaleditor{Amin Shokrollahi}{EPF Lausanne}
\journaleditor{Yossef Steinberg}{Technion}
\journaleditor{Wojciech Szpankowski}{Purdue University}
\journaleditor{David Tse}{Stanford University}
\journaleditor{Antonia Tulino}{Bell Labs}
\journaleditor{R\"{u}diger Urbanke}{EPF Lausanne}
\journaleditor{Emanuele Viterbo}{Monash University}
\journaleditor{Frans Willems}{TU Eindhoven}
\journaleditor{Raymond Yeung}{CUHK}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CIT-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{CITcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {CITcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Communications and Information Theory}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CIT}
\journalurl        {http://www.nowpublishers.com/CIT}
\journalissnprint  {1567-2190}
\journalissnonline {1567-2328 }
\journaldoi        {10.1561/01}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Communications and Information Theory publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Coded modulation}
\item{Coding theory and practice}
\item{Communication complexity}
\item{Communication system design}
\item{Cryptology and data security}
\item{Data compression}
\item{Data networks}
\item{Demodulation and Equalization}
\item{Denoising}
\item{Detection and estimation}
\item{Information theory and statistics}
\item{Information theory and computer science}
\item{Joint source/channel coding}
\item{Modulation and signal design}
\item{Multiuser detection}
\item{Multiuser information theory}
\item{Optical communication channels}
\item{Pattern recognition and learning}
\item{Quantization}
\item{Quantum information processing}
\item{Rate-distortion theory}
\item{Shannon theory}
\item{Signal processing for communications}
\item{Source coding}
\item{Storage and recording codes}
\item{Speech and Image Compression}
\item{Wireless Communications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Communications and Information Theory, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CIT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Fundamentals of Index Coding}\\
Fatemeh Arbabjolfaei and Young-Han Kim\\
ISBN: 978-1-68083-492-5\\
\\
\noindent \textit{Community Detection and Stochastic Block Models}\\
Emmanuel Abbe\\
ISBN: 978-1-68083-476-5\\
\\
\noindent \textit{Redundancy of Lossless Data Compression for Known Sources by Analytic Methods}\\
Michael Drmota and Wojciech Szpankowski\\
ISBN: 978-1-68083-284-6\\
\\
\noindent \textit{Multiterminal Secrecy by Public Discussion}\\
Prakash Narayan and Himanshu Tyagi\\
ISBN: 978-1-68083-186-3\\
\\
\noindent \textit{Channel Coding Methods for Non-Volatile Memories}\\
Lara Dolecek and Frederic Sala \\
ISBN: 978-1-68083-102-3

==> journaldata/DBS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Joseph M. Hellerstein}{University of California at Berkeley\\United States}
\journalchiefeditor{Surajit Chaudhuri}{Microsoft Research, Redmond\\United States}



\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Azza Abouzied}{NYU-Abu Dhabi}
\journaleditor{Gustavo Alonso}{ETH Zurich}
\journaleditor{Mike Cafarella}{University of Michigan}
\journaleditor{Alan Fekete}{University of Sydney}
\journaleditor{Ihab Ilyas}{University of Waterloo}
\journaleditor{Andy Pavlo}{Carnegie Mellon University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/DBS-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{DBScolor}{officegreen}   %new color names can be defined before use
\journalcolor      {DBScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Databases}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {DBS}
\journalurl        {http://www.nowpublishers.com/DBS}
\journalissnprint  {1931-7883}
\journalissnonline {1931-7891}
\journaldoi        {10.1561/19}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Databases publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Data Models and Query Languages}
    \item{Query Processing and Optimization}
    \item{Storage, Access Methods, and Indexing}
    \item{Transaction Management, Concurrency Control and Recovery}
    \item{Deductive Databases}
    \item{Parallel and Distributed Database Systems}
    \item{Database Design and Tuning}
    \item{Metadata Management}
    \item{Object Management}
    \item{Trigger Processing and Active Databases}
    \item{Data Mining and OLAP}
    \item{Approximate and Interactive Query Processing}
    \item{Data Warehousing}
    \item{Adaptive Query Processing}
    \item{Data Stream Management}
    \item{Search and Query Integration}
    \item{XML and Semi-Structured Data}
    \item{Web Services and Middleware}
    \item{Data Integration and Exchange}
    \item{Private and Secure Data Management}
    \item{Peer-to-Peer, Sensornet and Mobile Data Management}
    \item{Scientific and Spatial Data Management}
    \item{Data Brokering and Publish/Subscribe}
    \item{Data Cleaning and Information Extraction}
    \item{Probabilistic Data Management}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Databases, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/DBS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Data Infrastructure for Medical Research}\\
Thomas Heinis and Anastasia Ailamaki\\
ISBN: 978-1-68083-348-5\\
\\
\noindent \textit{Main Memory Database Systems}\\
Franz Faerber, Alfons Kemper, Per-Ake Larson, Justin Levandoski, Thomas Neumann and Andrew Pavlo\\
ISBN: 978-1-68083-324-9\\
\\
\noindent \textit{Query Processing on Probabilistic Data: A Survey}\\
Guy Van den Broeck and Dan Suciu\\
ISBN: 978-1-68083-314-0\\
\\
\noindent \textit{Big Graph Analytics Platforms}\\
Da Yan, Yingyi Bu, Yuanyuan Tian and Amol Deshpande\\
978-1-68083-242-6

==> journaldata/ECO-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{William H. Greene}{New York University\\United States}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Manuel Arellano}{CEMFI Spain}
\journaleditor{Wiji Arulampalam}{University of Warwick}
\journaleditor{Orley Ashenfelter}{Princeton University}
\journaleditor{Jushan Bai}{Columbia University}
\journaleditor{Badi Baltagi}{Syracuse University}
\journaleditor{Anil Bera}{University of Illinois}
\journaleditor{Tim Bollerslev}{Duke University}
\journaleditor{David Brownstone}{UC Irvine}
\journaleditor{Xiaohong Chen}{Yale University}
\journaleditor{Steven Durlauf}{University of Wisconsin}
\journaleditor{Amos Golan}{American University}
\journaleditor{Bill Griffiths}{University of Melbourne}
\journaleditor{James Heckman}{University of Chicago}
\journaleditor{Jan Kiviet}{University of Amsterdam}
\journaleditor{Gary Koop}{The University of Strathclyde}
\journaleditor{Michael Lechner}{University of St. Gallen}
\journaleditor{Lung-Fei Lee}{Ohio State University}
\journaleditor{Larry Marsh}{Notre Dame University}
\journaleditor{James MacKinnon}{Queens University}
\journaleditor{Bruce McCullough}{Drexel University}
\journaleditor{Jeff Simonoff}{New York University}
\journaleditor{Joseph Terza}{Purdue University}
\journaleditor{Ken Train}{UC Berkeley}
\journaleditor{Pravin Travedi}{Indiana University}
\journaleditor{Adonis Yatchew}{University of Toronto}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ECO-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ECOcolor}{brickred}   %new color names can be defined before use
\journalcolor      {ECOcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Econometrics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ECO}
\journalurl        {http://www.nowpublishers.com/ECO}
\journalissnprint  {1551-3076}
\journalissnonline {1551-3084}
\journaldoi        {10.1561/08}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Econometrics publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Econometric Models}
    \item{Simultaneous Equation Models}
    \item{Estimation Frameworks}
    \item{Biased Estimation}
    \item{Computational Problems}
    \item{Microeconometrics}
    \item{Treatment Modeling}
    \item{Discrete Choice Modeling}
    \item{Models for Count Data}
    \item{Duration Models}
   \item{Limited Dependent Variables}
    \item{Panel Data}
    \item{Time Series Analysis}
    \item{Latent Variable Models}
    \item{Qualitative Response Models}
    \item{Hypothesis Testing}
    \item{Econometric Theory}
    \item{Financial Econometrics}
    \item{Measurement Error in Survey Data}
    \item{Productivity Measurement and Analysis}
    \item{Semiparametric and Nonparametric Estimation}
    \item{Bootstrap Methods}
    \item{Nonstationary Time Series}
    \item{Robust Estimation}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Econometrics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ECO-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Data Visualization and Health Econometrics}\\
Andrew M. Jones\\
ISBN: 978-1-68083-318-8\\
\\
\noindent \textit{Spatial Econometrics: A Broad View}\\
Giuseppe Arbia\\
ISBN: 978-1-68083-172-6\\
\\
\noindent \textit{Bifurcation of Macroeconometric Models and Robustness of\\ Dynamical Inferences}\\
William A. Barnett\\
ISBN: 978-1-68083-046-0

==> journaldata/EDA-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Radu Marculescu}{Carnegie Mellon University}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Robert K. Brayton}{University of California, Berkeley}
\journaleditor{Raul Camposano}{Sage Design Atomation}
\journaleditor{K.T. Tim Cheng}{HKUST}
\journaleditor{Jason Cong}{University of California, Los Angeles}
\journaleditor{Masahiro Fujita}{University of Tokyo}
\journaleditor{Georges Gielen}{KU Leuven}
\journaleditor{Tom Henzinger}{IST Austria}
\journaleditor{Andrew Kahng}{University of California, San Diego}
\columnbreak
\journaleditor{Andreas Kuehlmann}{Synopsys}
\journaleditor{Sharad Malik}{Princeton University}
\journaleditor{Joel Phillips}{Cadence Berkeley Labs}
\journaleditor{Jonathan Rose}{University of Toronto}
\journaleditor{Rob Rutenbar}{University of Pittsburgh}
\journaleditor{Alberto Sangiovanni-Vincentelli}{University of California, Berkeley}
\journaleditor{Leon Stok}{IBM Research}
\end{multicols*}
\end{editorialboard} 

==> journaldata/EDA-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{EDAcolor}{brickred}   %new color names can be defined before use
\journalcolor      {EDAcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electronic Design Automation}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EDA}
\journalurl        {http://www.nowpublishers.com/EDA}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electronic Design Automation publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{System Level Design}
    \item{Behavioral Synthesis}
    \item{Logic Design}
    \item{Verification}
    \item{Test}
    \item{Physical Design}
    \item{Circuit Level Design}
    \item{Reconfigurable Systems}
    \item{Analog Design}
    \item{Embedded software and parallel programming}
   \item{Multicore, GPU, FPGA, and heterogeneous systems}
    \item{Distributed, networked embedded systems}
    \item{Real-time and cyberphysical systems}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Electronic Design Automation, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EDA-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Error-Efficient Computing Systems}\\
Phillip Stanley-Marbell and Martin Rinard\\
ISBN: 978-1-68083-358-4\\
\\
\noindent \textit{Secure Processors Part II: Intel SGX Security Analysis\\ and MIT Sanctum Architecture}\\
Victor Costan, Ilia Lebedev and Srinivas Devadas\\
ISBN: 978-1-68083-302-7\\
\\
\noindent \textit{Secure Processors Part I: Background, Taxonomy for Secure Enclaves\\ and Intel SGX Architecture}\\
Victor Costan, Ilia Lebedev and Srinivas Devadas\\
ISBN: 978-1-68083-300-3

==> journaldata/EES-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Marija D. Ili\'c}{Carnegie Mellon University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Istv\'an Erlich}{University of Duisburg-Essen}
\journaleditor{David Hill}{University of Hong Kong and University of Sydney}
\journaleditor{Daniel Kirschen}{University of Washington}
\journaleditor{J. Zico Kolter}{Carnegie Mellon University}
\journaleditor{Chao Lu}{Tsinghua University}
\journaleditor{Steven Low}{California Institute of Technology}
\journaleditor{Ram Rajagopa}{Stanford University}
\journaleditor{Lou van der Sluis}{TU Delft}
\journaleditor{Goran Strbac}{Imperial College London}
\journaleditor{Robert J. Thomas}{Cornell University}
\journaleditor{David Tse}{University of California, Berkeley}
\journaleditor{Le Xie}{Texas A\&M University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/EES-journaldata.tex <==
\definecolor{cinnabar}{rgb}{0.89, 0.26, 0.2}
\colorlet{EEScolor}{cinnabar}   %new color names can be defined before use
\journalcolor      {EEScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electric Energy Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EES}
\journalurl        {http://www.nowpublishers.com/EES}
\journalissnprint  {2332-6557}
\journalissnonline {2332-6565}
\journaldoi        {10.1561/31}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electric Energy Systems publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Advances in power dispatch}
\item{Demand-side and grid scale data analytics}
\item{Design and optimization of electric services}
\item{Distributed control and optimization of distribution networks}
\item{Distributed sensing for the grid}
\item{Distribution systems}
\item{Fault location and service restoration}
\item{Integration of physics-based and data-driven modeling of future electric energy systems}
\item{Integration of Power electronics, Networked FACTS}
\item{Integration of renewable energy sources}
\item{Interdependence of power system operations and planning and the electricity markets}
\item{Microgrids}
\item{Modern grid architecture}
\item{Power system analysis and computing}
\item{Power system dynamics}
\item{Power system operation}
\item{Power system planning}
\item{Power system reliability}
\item{Power system transients}
\item{Security and privacy}
\item{Stability and control for the whole multi-layer (granulated) network with new load models (to include storage, DR, EVs) and new generation}
\item{System protection and control}
\item{The new stability guidelines and control structures for supporting high penetration of renewables (>50\%)}
\item{Uncertainty quantification for the grid}
\item{System impacts of HVDC}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Electric Energy Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EES-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Sustainable Transportation with Electric Vehicles}\\
Fanxin Kong and Xue Liu\\
ISBN: 978-1-68083-388-1\\
\\
\noindent \textit{Unit Commitment in Electric Energy Systems}\\
Miguel F. Anjos and Antonio J. Conejo\\
ISBN: 978-1-68083-370-6\\
\\
\noindent \textit{Reliability Standards for the Operation and Planning of Future\\ Electricity Networks}\\
Goran Strbac, Daniel Kirschen and Rodrigo Moreno\\
ISBN: 978-1-68083-182-5\\
\\
\noindent \textit{Toward a Unified Modeling and Control for Sustainable and Resilient Electric Energy Systems}\\
Marija D. Ilic\\
ISBN: 978-1-68083-226-6

==> journaldata/ENT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}
\journalchiefeditor{David B. Audretsch}{Indiana University\\United States}\\
\journalchiefeditor{Mike Wright}{Imperial College London\\United Kingdom}
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Howard Aldrich}{University of North Carolina}
\journaleditor{Sharon Alvarez}{University of Denver}
\journaleditor{Per Davidsson}{Queensland University of Technology}
\journaleditor{Michael Frese}{National University of Singapore}
\journaleditor{William B. Gartner}{Copenhagen Business School}
\journaleditor{Magnus Henrekson}{IFN Stockholm}
\journaleditor{Michael A. Hitt}{Texas A\&M University}
\journaleditor{Joshua Lerner}{Harvard University}
\columnbreak
\journaleditor{Jeff McMullen}{Indiana University}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Maria Minniti}{Syracuse University}
\journaleditor{Simon Parker}{University of Western Ontario}
\journaleditor{Holger Patzelt}{TU Munich}
\journaleditor{Saras Sarasvathy}{University of Virginia}
\journaleditor{Roy Thurik}{Erasmus University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ENT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{ENTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {ENTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Entrepreneurship}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ENT}
\journalurl        {http://www.nowpublishers.com/ENT}
\journalissnprint  {1551-3114}
\journalissnonline {1551-3122}
\journaldoi        {10.1561/03}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Entrepreneurship publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Nascent and start-up entrepreneurs}
\item{Opportunity recognition}
\item{New venture creation process}
\item{Business formation}
\item{Firm ownership}
\item{Market value and firm growth}
\item{Franchising}
\item{Managerial characteristics and behavior of entrepreneurs}
\item{Strategic alliances and networks}
\item{Government programs and public policy}
\item{Gender and ethnicity}
\columnbreak
\item{New business financing:}
	\begin{itemize}
\item{Business angels}
\item{Bank financing, debt, and trade credit}
\item{Venture capital and private equity capital}
\item{Public equity and IPOs} 
\end{itemize}
\item{Family-owned firms}
\item{Management structure, governance and performance}
\item{Corporate entrepreneurship}
\item{High technology:}
	\begin{itemize}
        \item{Technology-based new firms}
        \item{High-tech clusters}
        \end{itemize}
\item{Small business and economic growth}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Entrepreneurship, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ENT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Knowledge-Intensive Innovative Entrepreneurship}\\
Franco Malerba and Maureen McKelvey\\
ISBN: 978-1-68083-518-2\\
\\
\noindent \textit{Senior Entrepreneurship: A Selective Review and a Research Agenda}\\
Catarina Seco Matos, Miguel Amaral and Rui Baptista\\
ISBN: 978-1-68083-504-5\\
\\
\noindent \textit{Contextual Entrepreneurship: An Interdisciplinary Perspective}\\
Ted Baker and Friederike Welter\\
ISBN: 978-1-68083-456-7\\
\\
\noindent \textit{Personality Traits of Entrepreneurs: A Review of Recent Literature}\\
Sari Pekkala Kerr, William R. Kerr and Tina Xu\\
ISBN: 978-1-68083-448-2\\
\\
\noindent \textit{Impact: Stanford University’s Economic Impact via Innovation and Entrepreneurship}\\
Charles E. Eesley and William F. Miller\\
ISBN: 978-1-68083-422-2\\
\\
\noindent \textit{Venture Capital, Angel Financing, and Crowdfunding of Entrepreneurial Ventures: A Literature Review}\\
Johannes Wallmeroth, Peter Wirtz and Alexander Peter Groh\\
ISBN: 978-1-68083-394-2

==> journaldata/FIN-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Sheridan Titman}{University of Texas at Austin\\United States}
\end{multicols}

\subsection{Associate Editors}
\begin{multicols}{1}
\journaleditor{Josef Zechner}{WU Vienna University of Economics and Finance}
\journaleditor{Chester Spatt}{Carnegie Mellon University}
\end{multicols}
\end{editorialboard} 

==> journaldata/FIN-journaldata.tex <==
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\colorlet{FINcolor}{ceruleanblue}   %new color names can be defined before use
\journalcolor      {FINcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Finance}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {FIN}
\journalurl        {http://www.nowpublishers.com/FIN}
\journalissnprint  {1567-2395}
\journalissnonline {1567-2409}
\journaldoi        {10.1561/05}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Finance publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Corporate Finance}
\begin{itemize}
\item{Corporate Governance}
\item{Corporate Financing}
\item{Dividend Policy and Capital Structure}
\item{Corporate Control}
\item{Investment Policy}
\item{Agency Theory and Information}
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Financial Markets}
\begin{itemize}
\item{Market Microstructure}
\item{Portfolio Theory}
\item{Financial Intermediation}
\item{Investment Banking}
\item{Market Efficiency}
\item{Security Issuance}
\item{Anomalies and Behavioral Finance}
\end{itemize}
\end{itemize}
\end{multicols}
%}
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
%\columnbreak
%\begin{itemize}
\item{Asset Pricing}
\begin{itemize}
\item{Asset-Pricing Theory}
\item{Asset-Pricing Models}
\item{Tax Effects}
\item{Liquidity} 
\item{Equity Risk Premium} 
\item{Pricing Models and Volatility} 
\item{Fixed Income Securities} 
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Derivatives}
\begin{itemize}
\item{Computational Finance}
\item{Futures Markets and Hedging}
\item{Financial Engineering}
\item{Interest Rate Derivatives}
\item{Credit Derivatives}
\item{Financial Econometrics}
\item{Estimating Volatilities and Correlations}
\end{itemize}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Finance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/FIN-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Initial Public Offerings: A Synthesis of the Literature and Directions for Future Research}\\
Michelle Lowry, Roni Michaely and Ekaterina Volkova\\
ISBN: 978-1-68083-340-9\\

\noindent \textit{Privatization, State Capitalism, and State Ownership of Business in the 21st Century}\\
William L. Megginson\\
ISBN: 978-1-68083-338-6\\

\noindent \textit{Executive Compensation}\\
Raghavendra Rau\\
ISBN: 978-1-68083-296-9\\
\\
\noindent \textit{Three Branches of Theories of Financial Crises}\\
Itay Goldstein and Assaf Razin\\
ISBN: 978-1-68083-084-2\\
\\
\noindent \textit{The Economics and Finance of Hedge Funds: A Review of the\\ Academic Literature}\\
Vikas Agarwal, Kevin A. Mullally, and Narayan Y. Naik\\
ISBN: 978-1-68083-156-6\\

==> journaldata/HCI-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Desney S. Tan}{Microsoft Research}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Ben Bederson}{University of Maryland}
\journaleditor{Sheelagh Carpendale}{University of Calgary}
\journaleditor{Andy Cockburn}{University of Canterbury}
\journaleditor{Jon Froehlich}{University of Washington}
\journaleditor{Juan Pablo Hourcade}{University of Iowa}
\journaleditor{Karrie Karahalios}{University of Illinois at Urbana-Champaign}
\journaleditor{Youn-Kyung Lim}{Korea Advanced Institute of Science and Technology}
\journaleditor{Nuria Oliver}{Telefonica}
\journaleditor{Orit Shaer}{Wellesley College}
\journaleditor{Kentaro Toyama}{University of Michigan}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/HCI-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{HCIcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {HCIcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Human-Computer Interaction}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {HCI}
\journalurl        {http://www.nowpublishers.com/HCI}
\journalissnprint  {1551-3955}
\journalissnonline {1551-3963}
\journaldoi        {10.1561/11}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Human-Computer Interaction publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{History of the research community}
\item{Theory}
\item{Technology}
\item{Computer Supported Cooperative Work}
\item{Interdisciplinary influence}
\item{Advanced topics and trends}
\end{itemize}
%\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Human-Computer Interaction, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/HCI-seriespage.tex <==
\vspace{12pt}
\noindent \textit{HCIs Making Agendas}\\
Jeffrey Bardzell, Shaowen Bardzell, Cindy Lin, Silvia Lindtner and Austin Toombs\\
ISBN: 978-1-68083-372-0\\
\\
\noindent \textit{A Survey of Value Sensitive Design Methods}\\
Batya Friedman, David G. Hendry and Alan Borning\\
ISBN: 978-1-68083-290-7\\
\\
\noindent \textit{Communicating Personal Genomic Information to Non-experts:\\ A New Frontier for Human-Computer Interaction}\\
Orit Shaer, Oded Nov, Lauren Westendorf and Madeleine Ball\\
ISBN: 978-1-68083-254-9\\
\\
\noindent \textit{Personal Fabrication}\\
Patrick Baudisch and Stefanie Mueller \\
ISBN: 978-1-68083-258-7\\
\\
\noindent \textit{Canine-Centered Computing}\\
Larry Freil, Ceara Byrne, Giancarlo Valentin, Clint Zeagler,\\ David Roberts, Thad Starner and Melody Jackson\\
ISBN: 978-1-68083-244-0\\
\\
\noindent \textit{Exertion Games}\\
Florian Mueller, Rohit Ashok Khot, Kathrin Gerling and\\ Regan Mandryk\\
ISBN: 978-1-68083-202-0

==> journaldata/INR-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Maarten de Rijke}{University of Amsterdam\\The Netherlands}
\journalchiefeditor{Yiqun Liu}{Tsinghua University\\China}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Barbara Poblete}{University of Chile}
\journaleditor{Claudia Hauff}{Delft University of Technology}
\journaleditor{Diane Kelly}{University of Tennessee}
\journaleditor{Doug Oard}{University of Maryland}
\journaleditor{Ellen M. Voorhees}{National Institute of Standards and Technology}
\journaleditor{Fabrizio Sebastiani}{Consiglio Nazionale delle Ricerche, Italy}
\journaleditor{Hang Li}{Bytedance Technology}
\journaleditor{Helen Huang}{University of Queensland}
\journaleditor{Ian Ruthven}{University of Strathclyde, Glasgow}
\journaleditor{Jaap Kamps}{University of Amsterdam}
\journaleditor{Jian-Yun Nie}{Universit{\'e} de Montreal}
\columnbreak
\journaleditor{Jimmy Lin}{University of Maryland}
\journaleditor{Leif Azzopardi}{University of Glasgow}
\journaleditor{Lynda Tamine}{University of Toulouse}
\journaleditor{Mark Sanderson}{RMIT University}
\journaleditor{Rodrygo Luis Teodoro Santos}{Universidade Federal de Minas Gerais}
\journaleditor{Ryen White}{Microsoft Research}
\journaleditor{Shane Culpepper}{RMIT}
\journaleditor{Soumen Chakrabarti}{Indian Institute of Technology}
\journaleditor{Tie-Yan Liu}{Microsoft Research}
\journaleditor{Xuanjing Huang}{Fudan University}
\journaleditor{Zi Helen Huang}{University of Queensland}
\end{multicols*}
\end{editorialboard} 

==> journaldata/INR-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{INRcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {INRcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Retrieval}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {INR}
\journalurl        {http://www.nowpublishers.com/INR}
\journalissnprint  {1554-0669}
\journalissnonline {1554-0677}
\journaldoi        {10.1561/15}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Retrieval publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Applications of IR}
\item{Architectures for IR}
\item{Collaborative filtering and recommender systems}
\item{Cross-lingual and multilingual IR}
\item{Distributed IR and federated search}
\item{Evaluation issues and test collections for IR}
\item{Formal models and language models for IR}
\item{IR on mobile platforms}
\item{Indexing and retrieval of structured documents}
\item{Information categorization and clustering}
\item{Information extraction}
\item{Information filtering and routing}
\item{Metasearch, rank aggregation and data fusion}
\item{Natural language processing for IR}
\item{Performance issues for IR systems, including algorithms, data structures, optimization techniques, and scalability}
\item{Question answering}
\item{Summarization of single documents, multiple documents, and corpora}
\item{Text mining}
\item{Topic detection and tracking}
\item{Usability, interactivity, and visualization issues in IR}
\item{User modelling and user studies for IR}
\item{Web search}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Retrieval, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 5 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/INR-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Efficient Query Processing for Scalable Web Search}\\
Nicola Tonellotto, Craig Macdonald and Iadh Ounis\\
ISBN: 978-1-68083-542-7\\

\noindent \textit{Geographic Information Retrieval: Progress and Challenges in Spatial Search of Text}\\
Ross S. Purves, Paul Clough, Christopher B. Jones, Mark H. Hall and\\ Vanessa Murdock\\
ISBN: 978-1-68083-412-3\\

\noindent \textit{Web Forum Retrieval and Text Analytics: A Survey}\\
Doris Hoogeveen, Li Wang, Timothy Baldwin and Karin M. Verspoor\\
ISBN: 978-1-68083-350-8

==> journaldata/ISY-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{Joey George}{Iowa State University\\United States}
%\end{multicols}

\subsection{Honorary Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Izak Benbasat}{University of British Columbia}
\journaleditor{Alan R. Dennis}{Kelley School of Business, Indiana University}
\journaleditor{Jacqueline Rees Ulmer}{Iowa State University}
\journaleditor{Veda Storey}{Georgia State University}
\journaleditor{Detmar Straub}{Georgia State University}
\journaleditor{Hugh Watson}{University of Georgia}
%\end{multicols*}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Alan Hevner}{University of South Florida}
\journaleditor{David Paradice}{Auburn University}
\journaleditor{Carol Saunders}{University of Central Florida}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ISY-journaldata.tex <==
\definecolor{regalia}{rgb}{0.32, 0.18, 0.5}
\colorlet{ISYcolor}{regalia}   %new color names can be defined before use
\journalcolor      {ISYcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ISY}
\journalurl        {http://www.nowpublishers.com/ISY}
\journalissnprint  {2331-1231}
\journalissnonline {2331-124X}
\journaldoi        {10.1561/29}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Systems publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{IS and Individuals}
\item{IS and Groups}
\item{IS and Organizations}
\item{IS and Industries}
\item{IS and Society}
\item{IS Development}
\item{IS Economics}
\item{IS Management}
\item{IS Research Methods}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ISY-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Enterprise Personal Analytics: The Next Frontier in Individual\\ Information Systems Research}\\
T. Clohessy, T. Acton, E. Whelan and W. Golden\\
ISBN: 978-1-68083-460-4\\
\\
\noindent \textit{Empirical Research in Information Systems: 2001–2015}\\
S. Shuraida, H. Barki and A. Luong\\
ISBN: 978-1-68083-430-7\\
\\
\noindent \textit{A Review of Ethical Issue Considerations in the Information\\ Systems Research Literature}\\
D. Paradice, D. Freeman, J. Hao, J. Lee and D. Hall\\
ISBN: 978-1-68083-398-0\\
\\
\noindent \textit{Information Systems Success Measurement}\\
W. H. DeLone and E. R. McLean\\
ISBN: 978-1-68083-142-9

==> journaldata/MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{Toyota Technological Institute}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Northeastern University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Amazon}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{Yale}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{KU Leuven}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Microsoft Research}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Non-convex Optimization for Machine Learningy}\\
Prateek Jain and Purushottam Ka\\
ISBN: 978-1-68083-368-3\\
\\
\noindent \textit{Kernel Mean Embedding of Distributions: A Review and Beyond}\\
Krikamol Muandet, Kenji Fukumizu, Bharath Sriperumbudur and\\ Bernhard Scholkopf\\
ISBN: 978-1-68083-288-4\\
\\
\noindent \textit{Tensor Networks for Dimensionality Reduction and Large-scale\\ Optimization: Part 1 Low-Rank Tensor Decompositions}\\
Andrzej Cichocki, Anh-Huy Phan, Qibin Zhao, Namgil Lee,\\ Ivan Oseledets, Masashi Sugiyama and Danilo P. Mandic\\
ISBN: 978-1-68083-222-8\\
\\
\noindent \textit{Tensor Networks for Dimensionality Reduction and Large-scale\\ Optimization: Part 2 Applications and Future Perspectives}\\
Andrzej Cichocki, Anh-Huy Phan, Qibin Zhao, Namgil Lee,\\ Ivan Oseledets, Masashi Sugiyama and Danilo P. Mandic\\
ISBN: 978-1-68083-276-1\\
\\
\noindent \textit{Patterns of Scalable Bayesian Inference}\\
Elaine Angelino, Matthew James Johnson and Ryan P. Adams \\
ISBN: 978-1-68083-218-1\\
\\
\noindent \textit{Generalized Low Rank Models}\\
Madeleine Udell, Corinne Horn, Reza Zadeh and Stephen Boyd \\
ISBN: 978-1-68083-140-5

==> journaldata/MGT-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{2}\raggedright
\journalchiefeditor{Nicholas S. Argyres}{Olin Business School, Washington University\\United States}
\journalchiefeditor{Timothy M. Devinney}{Leeds University Business School\\United Kingdom}
\journalchiefeditor{James Campbell Quick}{The University of Texas at Arlington\\United States}
\end{multicols}

\subsection{Editors}
\begin{multicols}{3}\raggedright \raggedcolumns
\renewcommand\journaleditor[2]{\par\textbf{#1}\\#2}%
\subsubsection{\footnotesize International Business}

\journaleditor{Gabriel R.G. Benito}{BI Norwegian School of Management}
\journaleditor{Allan Bird}{Northeastern University}
\journaleditor{Julian Birkinshaw}{London Business School}
\journaleditor{Peter Buckley}{University of Leeds}
\journaleditor{Saul Estrin}{London School of Economics}
\journaleditor{Sarianna Lundin}{University of Bremen}
\journaleditor{Xavier Martin}{Tilburg University} 
\journaleditor{Ram Mudambi}{Temple University}

\columnbreak

\subsubsection{\footnotesize Organizational Behavior}

\journaleditor{Myrtle Bell}{University of Texas at Arlington}
\journaleditor{Cary Cooper}{Lancaster University}
\journaleditor{Richard Griffin}{Texas A\&M University}
\journaleditor{Sean Hannah}{Wake Forest University}
\journaleditor{Debra Nelson}{Oklahoma State University}
\journaleditor{Pamela Perrewe}{Florida State University}

\columnbreak

\subsubsection{\footnotesize Strategy}

\journaleditor{Rajshree Agarwal}{University of Maryland}
\journaleditor{Marvin Lieberman}{UCLA}) 
\journaleditor{Michael Lenox}{University of Virginia}
\journaleditor{Joseph Mahoney}{University of Illinois at Urbana-Champaign}
\journaleditor{Jesper Sørensen}{Stanford University}
\journaleditor{Olav Sorenson}{Yale University}
\end{multicols}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MGT-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{MGTcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {MGTcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MGT}
\journalurl        {http://www.nowpublishers.com/MGT}
\journalissnprint  {2475-6946}
\journalissnonline {2475-6954}
\journaldoi        {10.1561/34}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management publishes
 survey and tutorial articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{International Business}
\item{Organizational Behavior}
\item{Strategic Management}
\end{itemize}
 %\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-editorialboard.tex <==
%MIC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{W. Kip Viscusi}{Vanderbilt University Law School\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Richard Carson}{University of California, San Diego}
\journaleditor{William Gentry}{Williams College}
\journaleditor{Tom Kniesner}{Syracuse University}
\journaleditor{Mark V. Pauly}{University of Pennsylvania}
\journaleditor{Yossi Spiegel}{Tel Aviv University}
\journaleditor{William Zame}{University of California, Los Angeles}
\journaleditor{James Ziliak}{University of Kentucky}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MIC-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{MICcolor}{pinegreen}   %new color names can be defined before use   %new color names can be defined before use
\journalcolor      {MICcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Microeconomics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MIC}
\journalurl        {http://www.nowpublishers.com/MIC}
\journalissnprint  {1547-9846}
\journalissnonline {1547-9854}
\journaldoi        {10.1561/07}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Environmental economics}
\item{Health economics}
\item{Industrial organization}
\item{Labor economics}
\item{Law and economics}
\item{Public economics}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-seriespage.tex <==
\vspace{12pt}
\vspace{12pt}
\noindent \textit{Natural Gas Pipeline Regulation in the United States: Past, Present, and Future}\\
Matthew E. Oliver
\\ISBN: 978-1-68083-452-9
\\
\\
\noindent \textit{The U.S. Market for Uranium: 70 Years of History}\\
Charles F. Mason
\\ISBN: 978-1-68083-382-9
\\
\\
\noindent \textit{Game Theory and Water Resources: Critical Review of its Contributions, Progress and Remaining Challenges}\\
Ariel Dinar and Margaret Hogarth
\\ISBN: 978-1-68083-016-3


==> journaldata/MKT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Jehoshua Eliashberg}{University of Pennsylvania}

\subsection{Associate Editors}

\journaleditor{Bernd Schmitt}{Columbia University}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Gerrit van Bruggen}{Erasmus University}
\journaleditor{Christophe van den Bulte}{University of Pennsylvania}
\journaleditor{Amitava Chattopadhyay}{INSEAD}
\journaleditor{Pradeep Chintagunta}{University of Chicago}
\journaleditor{Dawn Iacobucci}{Vanderbilt University}
\journaleditor{Raj Ragunathan}{University of Texas, Austin}
\journaleditor{J. Miguel Villas-Boas}{University of California, Berkeley}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MKT-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MKTcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MKTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Marketing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MKT}
\journalurl        {http://www.nowpublishers.com/MKT}
\journalissnprint  {1555-0753}
\journalissnonline {1555-0761}
\journaldoi        {10.1561/17}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Marketing publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{B2B Marketing}
\item{Bayesian Models}
\item{Behavioral Decision Making}
\item{Branding and Brand Equity}
\item{Channel Management}
\item{Choice Modeling}
\item{Comparative Market Structure}
\item{Competitive Marketing Strategy}
\item{Conjoint Analysis}
\item{Customer Equity}
\item{Customer Relationship Management}
\item{Game Theoretic Models}
\item{Group Choice and Negotiation}
\item{Discrete Choice Models}
\item{Individual Decision Making}
\item{Marketing Decisions Models}
\item{Market Forecasting}
\item{Marketing Information Systems}
\item{Market Response Models}
\item{Market Segmentation}
\item{Market Share Analysis}
\item{Multi-channel Marketing}
\item{New Product Diffusion}
\item{Pricing Models}
\item{Product Development}
\item{Product Innovation}
\item{Sales Forecasting}
\item{Sales Force Management}
\item{Sales Promotion}
\item{Services Marketing}
\item{Stochastic Model}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Marketing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MKT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Modeling Dynamic Relations Among Marketing and Performance Metrics}\\
Koen H. Pauwels \\
ISBN:978-1-68083-490-1\\
\\
\noindent \textit{Sales Force Compensation: Trends and Research Opportunities}\\
Dominique Rouziès and Vincent Onyemah\\
ISBN: 978-1-68083-488-8\\
\\
\noindent \textit{From Doubt to Functionality: An Imagery Story}\\
Rashmi Adaval\\
ISBN:978-1-68083-458-1\\
\\
\noindent \textit{Consumer Informational Privacy}\\
Frank T. Beke, Felix Eggers and Peter C. Verhoef \\
ISBN: 978-1-68083-168-9


==> journaldata/NET-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Anthony Ephremides}{University of Maryland\\United States}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fran\c{c}ois Baccelli}{University of Texas, Austin}
\journaleditor{Victor Bahl}{Microsoft Research}
\journaleditor{Helmut B\"{o}lcskei}{ETH Zurich}
\journaleditor{J.J. Garcia-Luna Aceves}{UC Santa Cruz}
\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Roch Guerin}{Washington University in Saint Louis}
\journaleditor{Bruce Hajek}{UIUC}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Frank Kelly}{University of Cambridge}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Steven Low}{Caltech}
\journaleditor{Eytan Modiano}{MIT}
\columnbreak
\journaleditor{Keith Ross}{Polytechnic Institute of NYU}
\journaleditor{Henning Schulzrinne}{Columbia University}
\journaleditor{Mani Srivastava}{UCLA}
\journaleditor{Leandros Tassiulas}{Yale University}
\journaleditor{Lang Tong}{Cornell University}
\journaleditor{Ozan Tonguz}{Carnegie Mellon University}
\journaleditor{Don Towsley}{University of Massachusetts, Amherst}
\journaleditor{Nitin Vaidya}{UIUC}
\journaleditor{Pravin Varaiya}{UC Berkeley}
\journaleditor{Roy Yates}{Rutgers University}
\journaleditor{Raymond Yeung}{Chinese University of Hong Kong}
\end{multicols*}
\end{editorialboard} 

==> journaldata/NET-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{NETcolor}{cerise}   %new color names can be defined before use
\journalcolor      {NETcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Networking}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {NET}
\journalurl        {http://www.nowpublishers.com/NET}
\journalissnprint  {1554-057X}
\journalissnonline {1554-0588}
\journaldoi        {10.1561/13}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Networking publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Modeling and Analysis of:}
	\begin{itemize}
	\item{Ad Hoc Wireless Networks}
	\item{Sensor Networks}
	\item{Optical Networks}
	\item{Local Area Networks}
	\item{Satellite and Hybrid Networks}
	\item{Cellular Networks}
	\item{Internet and Web Services}
	\end{itemize}
\item{Protocols and Cross-Layer Design}
\item{Network Coding}
\item{Energy-Efficiency Incentives/Pricing/Utility-based}
\item{Games (co-operative or not)}
\item{Security}
\item{Scalability}
\item{Topology}
\item{Control/Graph-theoretic models}
\item{Dynamics and Asymptotic Behavior of Networks}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Networking, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/NET-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Age of Information: A New Concept, Metric, and Tool}\\
Antzela Kosta, Nikolaos Pappas and Vangelis Angelakis\\
ISBN: 978-1-68083-360-7\\
\\
\noindent \textit{Network and Protocol Architectures for Future Satellite Systems}\\
Tomaso de Cola, Alberto Ginesi, Giovanni Giambene,\\ George C. Polyzos, Vasilios A. Siris, Nikos Fotiou and Yiannis Thomas\\
ISBN: 978-1-68083-334-8\\
\\
\noindent \textit{Duality of the Max-Plus and Min-Plus Network Calculus}\\
Jorg Liebeherr\\
ISBN: 978-1-68083-294-5\\
\\
\noindent \textit{Opportunistic Routing in Wireless Networks}\\
Tara Javidi and Eric Van Buhler\\
ISBN: 978-1-68083-150-4

==> journaldata/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> journaldata/OPT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{Stephen P. Boyd}{Stanford University, USA}
\journalchiefeditor{Yinyu Ye}{Stanford University, USA}
\journalchiefeditor{Garud Iyengar}{Columbia University, USA}
%\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dimitris Bertsimas}{Massachusetts Institute of Technology}
\journaleditor{John R. Birge}{The University of Chicago}
\journaleditor{Robert E. Bixby}{Rice University}
\journaleditor{Emmanuel Candes}{Stanford University}
\journaleditor{David Donoho}{Stanford University}
\journaleditor{Laurent El Ghaoui}{University of California, Berkeley}
\journaleditor{Donald Goldfarb}{Columbia University}
\journaleditor{Michael I. Jordan}{University of California, Berkeley}
\journaleditor{Zhi-Quan (Tom) Luo}{University of Minnesota, Twin Cites}
\journaleditor{George L. Nemhauser}{Georgia Institute of Technology}
\journaleditor{Arkadi Nemirovski}{Georgia Institute of Technology}
\columnbreak
\journaleditor{Yurii Nesterov}{HSE University}
\journaleditor{Jorge Nocedal}{Northwestern University}
\journaleditor{Pablo A. Parrilo}{Massachusetts Institute of Technology}
\journaleditor{Boris T. Polyak}{Institute for Control Science, Moscow}
\journaleditor{Tam\'as Terlaky}{Lehigh University}
\journaleditor{Michael J. Todd}{Cornell University}
\journaleditor{Kim-Chuan Toh}{National University of Singapore}
\journaleditor{John N. Tsitsiklis}{Massachusetts Institute of Technology}
\journaleditor{Lieven Vandenberghe}{University of California, Los Angeles}
\journaleditor{Robert J. Vanderbei}{Princeton University}
\journaleditor{Stephen J. Wright}{University of Wisconsin}
\end{multicols*}
\end{editorialboard} 

==> journaldata/OPT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{OPTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {OPTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Optimization}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {OPT}
\journalurl        {http://www.nowpublishers.com/OPT}
\journalissnprint  {2167-3888}
\journalissnonline {2167-3918}
\journaldoi        {10.1561/24}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Optimization publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{algorithm design, analysis, and implementation (especially, on modern computing platforms}
\item{models and modeling systems, new optimization formulations for practical problems}
\item{applications of optimization in machine learning, statistics, and data analysis, signal and image processing, computational economics and finance, engineering design, scheduling and resource allocation, and other areas}
\end{itemize}
 %\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Optimization, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/OPT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{The Many Faces of Degeneracy in Conic Optimization}\\
Dmitriy Drusvyatskiy and Henry Wolkowicz\\
ISBN: 978-1-68083-390-4\\
\\
\noindent \textit{Multi-Period Trading via Convex Optimization}\\
Stephen Boyd, Enzo Busseti, Steve Diamond, Ronald N. Kahn,\\ Kwangmoo Koh, Peter Nystrup and Jan Speth \\
ISBN: 978-1-68083-298-3\\
\\
\noindent \textit{Introduction to Online Convex Optimization}\\
Elad Hazan\\
ISBN: 978-1-68083-170-2\\
\\
\noindent \textit{Low-Rank Semidefinite Programming: Theory and Applications}\\
Alex Lemon, Anthony Man-Cho So and Yinyu Ye\\
ISBN: 978-1-68083-136-8

==> journaldata/PGL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Mooly Sagiv}{Tel-Aviv University, Israel}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and UC Santa Cruz}
\journaleditor{Anindya Banerjeei}{IMDEA Software Instituet}
\journaleditor{Patrick Cousoti}{ENS, Paris and NYU}
\journaleditor{Oege De Moori}{University of Oxford}
\journaleditor{Matthias Felleiseni}{Northeastern University}
\journaleditor{John Fieldi}{Google}
\journaleditor{Cormac Flanagani}{UC Santa Cruz}
\journaleditor{Philippa Gardneri}{Imperial College}
\journaleditor{Andrew Gordoni}{Microsoft Research and University of Edinburgh}
\journaleditor{Dan Grossmani}{University of Washington}
\journaleditor{Robert Harper}{CMU}
\journaleditor{Tim Harris}{Amazon}
\journaleditor{Fritz Hengleini}{University of Copenhagen}
\journaleditor{Rupak Majumdari}{MPI and UCLA}
\journaleditor{Kenneth McMillani}{Microsoft Research}
\journaleditor{J. Eliot B. Mossi}{University of Massachusetts, Amherst}
\journaleditor{Andrew C. Myersi}{Cornell University}
\journaleditor{Hanne Riis Nielsoni}{Technical University of Denmark}
\journaleditor{Peter O'Hearni}{University College London}
\journaleditor{Benjamin C. Piercei}{University of Pennsylvania}
\journaleditor{Andrew Pittsi}{University of Cambridge}
\journaleditor{Ganesan Ramalingami}{Microsoft Research}
\journaleditor{Mooly Sagivi}{Tel Aviv University}
\journaleditor{Davide Sangiorgii}{University of Bologna}
\journaleditor{David Schmidti}{Kansas State University}
\journaleditor{Peter Sewelli}{University of Cambridge}
\journaleditor{Scott Stolleri}{Stony Brook University}
\journaleditor{Peter Stuckeyi}{University of Melbourne}
\journaleditor{Jan Viteki}{Northeastern University}
\journaleditor{Philip Wadleri}{University of Edinburgh}
\journaleditor{David Walkeri}{Princeton University}
\journaleditor{Stephanie Weirici}{University of Pennsylvania}
\end{multicols*}
\end{editorialboard} 

==> journaldata/PGL-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{PGLcolor}{brickred}   %new color names can be defined before use
\journalcolor      {PGLcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Programming Languages}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {PGL}
\journalurl        {http://www.nowpublishers.com/PGL}
\journalissnprint  {2325-1107}
\journalissnonline {2325-1131}
\journaldoi        {10.1561/25}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Programming Languages publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Abstract Interpretation}
\item{Compilation and Interpretation Techniques}
\item{Domain Specific Languages}
\item{Formal Semantics, including Lambda Calculi, Process Calculi, and Process Algebra}
\item{Language Paradigms}
    \item{Mechanical Proof Checking}
    \item{Memory Management}
    \item{Partial Evaluation}
    \item{Program Logic}
    \item{Programming Language Implementation}
    \item{Programming Language Security}
    \item{Programming Languages for Concurrency}
    \item{Programming Languages for Parallelism}
    \item{Program Synthesis}
    \item{Program Transformations and Optimizations}
    \item{Program Verification}
    \item{Runtime Techniques for Programming Languages}
    \item{Software Model Checking}
    \item{Static and Dynamic Program Analysis}
    \item{Type Theory and Type Systems}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Programming Languages, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/PGL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Tutorial on Static Inference of Numeric Invariants by Abstract\\ Interpretation}\\
Antoine Min\'e\\
ISBN: 978-1-68083-386-7\\
\\
\noindent \textit{Program Synthesis}\\
Sumit Gulwani, Oleksandr Polozov and Rishabh Singh\\
ISBN: 978-1-68083-292-1\\
\\
\noindent \textit{Programming with Big Code}\\
Martin Vechev and Eran Yahav\\
ISBN: 978-1-68083-230-3
\\
\\
\noindent \textit{Behavioral Types in Programming Languages}\\
Davide Ancona et al.\\
ISBN: 978-1-68083-134-4
\\
\\
\noindent \textit{Computer-Assisted Query Formulation}\\
Alvin Cheung and Armando Solar-Lezama\\
ISBN: 978-1-68083-036-1

==> journaldata/ROB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Henrik Christensen}{University of California, San Diego}
\journalchiefeditor{Roland Siegwart}{ETH Zurich}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Minoru Asada}{Osaka University}
\journaleditor{Antonio Bicchi}{University of Pisa}
\journaleditor{Aude Billard}{EPFL}
\journaleditor{Cynthia Breazeal}{Massachusetts Institute of Technology}
\journaleditor{Oliver Brock}{TU Berlin}
\journaleditor{Wolfram Burgard}{University of Freiburg}
\journaleditor{Udo Frese}{University of Bremen}
\journaleditor{Ken Goldberg}{University of California, Berkeley}
\journaleditor{Hiroshi Ishiguro}{Osaka University}
\journaleditor{Makoto Kaneko}{Osaka University}
\journaleditor{Danica Kragic}{KTH Stockholm}
\journaleditor{Vijay Kumar}{University of Pennsylvania}
\journaleditor{Simon Lacroix}{LAAS}
\journaleditor{Christian Laugier}{INRIA}
\journaleditor{Steve LaValle}{University of Illinois at Urbana-Champaign}
\journaleditor{Yoshihiko Nakamura}{The University of Tokyo}
\journaleditor{Brad Nelson}{ETH Zurich}
\journaleditor{Paul Newman}{University of Oxford}
\journaleditor{Daniela Rus}{Massachusetts Institute of Technology}
\journaleditor{Giulio Sandini}{University of Genova}
\journaleditor{Sebastian Thrun}{Stanford University}
\journaleditor{Manuela Veloso}{Carnegie Mellon University}
\journaleditor{Markus Vincze}{Vienna University}
\journaleditor{Alex Zelinsky}{DSTG}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ROB-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{ROBcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {ROBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Robotics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ROB}
\journalurl        {http://www.nowpublishers.com/ROB}
\journalissnprint  {1935-8253}
\journalissnonline {1935-8261}
\journaldoi        {10.1561/23}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Robotics publishes
 survey and tutorial articles in the following topics:
\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Mathematical modelling}
\item{Kinematics}
\item{Dynamics}
\item{Estimation Methods}
\item{Robot Control}
\item{Planning}
\item{Artificial Intelligence in Robotics}
\item{Software Systems and Architectures}
\item{Mechanisms and Actuators}
\item{Sensors and Estimation}
\item{Planning and Control}
\item{Human-Robot Interaction}
\item{Industrial Robotics}
\item{Service Robotics }
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Robotics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ROB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Energy in Robotics}\\
Gerrit A. Folkertsma and Stefano Stramigioli\\
ISBN: 978-1-68083-312-6\\
\\
\noindent \textit{Factor Graphs for Robot Perception}\\
Frank Dellaert and Michael Kaess\\
ISBN: 978-1-68083-326-3\\
\\
\noindent \textit{A Survey of Methods for Safe Human-Robot Interaction}\\
Przemyslaw A. Lasota, Terrence Fong and Julie A. Shah\\
ISBN: 978-1-68083-278-5\\
\\
\noindent \textit{Soft-Material Robotics}\\
Sangbae Kim and Patrick M. Wensing \\
ISBN: 978-1-68083-256-3\\
\\
\noindent \textit{Cyber-Maritime Cycle: Autonomy of Marine Robots for Ocean Sensing}\\
Fumin Zhang\\
ISBN: 978-1-68083-232-7

==> journaldata/SEC-editorialboard.tex <==
%SEC-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Anupam Datta}{Carnegie Mellon University, USA}
\journalchiefeditor{Jeannette Wing}{Columbia University, USA}


\subsection{Editors}
\begin{multicols}{2}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and University of California, Santa Cruz}
\journaleditor{Michael Backes}{Saarland University}
\journaleditor{Dan Boneh}{Stanford University, USA}
\journaleditor{V\'eronique Cortier}{LORIA, CNRS, France}
\journaleditor{Lorrie Cranor}{Carnegie Mellon University}
\journaleditor{C\'edric Fournet}{Microsoft Research}
\journaleditor{Virgil Gligor}{Carnegie Mellon University}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Deirdre Mulligan}{University of California, Berkeley}
\journaleditor{Andrew Myers}{Cornell University}
\journaleditor{Helen Nissenbaum}{New York University}
\journaleditor{Michael Reiter}{University of North Carolina}
\journaleditor{Shankar Sastry}{University of California, Berkeley}
\journaleditor{Dawn Song}{University of California, Berkeley}
\journaleditor{Daniel Weitzner}{Massachusetts Institute of Technology}
\end{multicols}
\end{editorialboard} 


==> journaldata/SEC-journaldata.tex <==
\definecolor{bananayellow}{rgb}{1.0, 0.88, 0.21}
\colorlet{SECcolor}{bananayellow}   %new color names can be defined before use
\journalcolor      {SECcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Privacy and Security}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SEC}
\journalurl        {http://nowpublishers.com/SEC}
\journalissnprint  {2474-1558}
\journalissnonline {2474-1566}
\journaldoi        {10.1561/33}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Privacy and Security publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Access control}
\item{Accountability}
\item{Anonymity}
\item{Application security}
\item{Artifical intelligence methods in security and privacy}
\item{Authentication}
\item{Big data analytics and privacy}
\item{Cloud security}
\item{Cyber-physical systems security and privacy}
\item{Distributed systems security and privacy}
\item{Embedded systems security and privacy}
\item{Forensics}
\item{Hardware security}
\item{Human factors in security and privacy}
\item{Information flow}
\item{Intrusion detection}
\item{Malware}
\item{Metrics}
\item{Mobile security and privacy}
\item{Language-based security and privacy}
\item{Network security}
\item{Privacy-preserving systems}
\item{Protocol security}
\item{Security and privacy policies}
\item{Security architectures}
\item{System security}
\item{Web security and privacy}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Privacy and Security, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SEC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Contextual Integrity through the Lens of Computer Science}\\
Sebastian Benthall, Seda Gurses and Helen Nissenbaum\\
ISBN: 978-1-68083-384-3\\
\\
\noindent \textit{Methods for Location Privacy: A comparative overview}\\
Kostantinos Chatzikokolakis, Ehab ElSalamouny, Catuscia Palamidessi and Pazii Anna\\
ISBN: 978-1-68083-366-9\\
\\
\noindent \textit{Principles and Implementation Techniques of Software-Based Fault Isolation}\\
Gang Tan\\
ISBN: 978-1-68083-344-7\\
\\
\noindent \textit{Modeling and Verifying Security Protocols with the Applied Pi\\ Calculus and ProVerif}\\
Bruno Blanchet\\
ISBN: 978-1-68083-206-8

==> journaldata/SIG-editorialboard.tex <==
%SIG-Editorialboard.

\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Yonina Eldar}{Weizmann Institute\\Israel}



\subsection{Editors}
\begin{multicols}{3}\raggedcolumns
\journaleditor{Pao-Chi Chang}{National Central University}
\journaleditor{Pamela Cosman}{University of California, San Diego}
\journaleditor{Michelle Effros}{California Institute of Technology}
\journaleditor{Yariv Ephraim}{George Mason University}
\journaleditor{Alfonso Farina}{Selex ES}
\journaleditor{Sadaoki Furui}{Tokyo Institute of Technology}
\journaleditor{Georgios Giannakis}{University of Minnesota}
\journaleditor{Vivek Goyal}{Boston University}
\journaleditor{Sinan Gunturk}{Courant Institute}
\journaleditor{Christine Guillemot}{INRIA}
\journaleditor{Robert W. Heath, Jr.}{The University of Texas at Austin}
\journaleditor{Sheila Hemami}{Northeastern University}
\journaleditor{Lina Karam}{Arizona State University}
\journaleditor{Nick Kingsbury}{University of Cambridge}
\journaleditor{Alex Kot}{Nanyang Technical University}
\journaleditor{Jelena Kovacevic}{Carnegie Mellon University}
\journaleditor{Geert Leus}{TU Delft}
\journaleditor{Jia Li}{Pennsylvania State University}
\journaleditor{Henrique Malvar}{Microsoft Research}
\journaleditor{B.S. Manjunath}{University of California, Santa Barbara}
\journaleditor{Urbashi Mitra}{University of Southern California}
\journaleditor{Bj\"{o}rn Ottersten}{KTH Stockholm}
\journaleditor{Vincent Poor}{Princeton University}
\journaleditor{Anna Scaglione}{University of California, Davis}
\journaleditor{Mihaela van der Shaar}{University of California, Los Angeles}
\journaleditor{Nicholas D. Sidiropoulos}{Technical University of Crete}
\journaleditor{Michael Unser}{EPFL}
\journaleditor{P.P. Vaidyanathan}{California Institute of Technology}
\journaleditor{Ami Wiesel}{The Hebrew University of Jerusalem}
\journaleditor{Min Wu}{University of Maryland}
\journaleditor{Josiane Zerubia}{INRIA}
\end{multicols}
\end{editorialboard} 


==> journaldata/SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SIG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Massive MIMO Networks: Spectral, Energy, and Hardware Efficiency}\\
Emil Bjornson, Jakob Hoydis and Luca Sanguinetti\\
ISBN: 978-1-68083-985-2\\
\\
\noindent \textit{Using Inertial Sensors for Position and Orientation Estimation}\\
Manon Kok, Jeroen D. Hol and Thomas B. Schon\\
ISBN: 978-1-68083-356-0\\
\\
\noindent \textit{Computational Visual Attention Models}\\
Milind S. Gide and Lina J. Karam\\
ISBN: 978-1-68083-280-8\\
\\
\noindent \textit{Video Coding: Part II of Fundamentals of Source and Video Coding}\\
Thomas Wiegand and Heiko Schwarz\\
ISBN: 978-1-68083-178-8

==> journaldata/STP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/STP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Panos J. Antsaklis}{University of Notre Dame\\United States}
\journalchiefeditor{Alessandro Astolfi}{Imperial College London, United Kingdom\\ University of Rome ''Tor Vergata'', Italy}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{John Baillieuli}{Boston University}
\journaleditor{Peter Caines}{McGill University}
\journaleditor{Christos Cassandras}{Boston University}
\journaleditor{Denis Dochain}{UC Louvain}
\journaleditor{Magnus Egerstedt}{Georgia Institute of Technology}
\journaleditor{Karl Henrik Johansson}{KTH Stockholm}
\journaleditor{Miroslav Krstic}{University of California, San Diego}
\journaleditor{Jan Maciejowski}{University of Cambridge}
\columnbreak
\journaleditor{Dragan Nesic}{The University of Melbourne}
\journaleditor{Marios Polycarpou}{University of Cyprus}
\journaleditor{J\"{o}rg Raisch}{Technical University Berlin}
\journaleditor{Arjan van der Schaft}{University of Groningen}
\journaleditor{M. Elena Valcher}{University of Padova}
\journaleditor{Richard Vinter}{Imperial College London}
\journaleditor{George Weiss}{Tel Aviv University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/SYS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet {SYScolor}{cobalt} %new color names can be defined before use
\journalcolor      {SYScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Systems and Control}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SYS}
\journalurl        {http://www.nowpublishers.com/SYS}
\journalissnprint  {2325-6818}
\journalissnonline {2325-6826}
\journaldoi        {10.1561/26}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Systems and Control publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Control of:}
	\begin{itemize}
	\item{Hybrid and Discrete Event Systems}
	\item{Nonlinear Systems}
	\item{Network Systems}
	\item{Stochastic Systems}
	\item{Multi-agent Systems}
	\item{Distributed Parameter Systems}
	\item{Delay Systems}
	\end{itemize}
\item{Filtering, Estimation, Identification}
\item{Optimal Control}
\item{Systems Theory}
\item{Control Applications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Systems and Control, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Economic Model Predictive Control}\\
Helen Durand and Panagiotis D. Christofides\\
ISBN: 978-1-68083-432-1\\
\\
\noindent \textit{Distributed Averaging and Balancing in Network Systems}\\
Christoforos N. Hadjicostis, Alejandro D. Dominguez-Garcia and\\ Themistokis Charalambous\\
ISBN: 978-1-68083-438-3\\
\\
\noindent \textit{Economic Nonlinear Model Predictive Control}\\
Timm Faulwasser, Lars Grune and Matthias A. Muller\\
ISBN: 978-1-68083-392-8


==> journaldata/TCS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Madhu Sudan}{Harvard University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Bernard Chazelle}{Princeton University}
\journaleditor{Oded Goldreich}{Weizmann Institute}
\journaleditor{Shafi Goldwasser}{Massachusetts Institute of Technology and Weizmann Institute}
\journaleditor{Sanjeev Khanna}{University of Pennsylvania}
\journaleditor{Jon Kleinberg}{Cornell University}
\journaleditor{L\'aszl\'o Lov\'asz}{Eötvös Lor\'and University}
\journaleditor{Christos Papadimitriou}{University of California, Berkeley}
\journaleditor{Peter Shor}{Massachusetts Institute of Technology}
\journaleditor{Eva Tardos}{Cornell University}
\journaleditor{Avi Wigderson}{AIS, Princeton University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TCS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{TCScolor}{cobalt}   %new color names can be defined before use
\journalcolor      {TCScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TCS}
\journalurl        {http://www.nowpublishers.com/TCS}
\journalissnprint  {1551-305X}
\journalissnonline {1551-3068}
\journaldoi        {10.1561/04}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Algorithmic game theory}
    \item{Computational algebra}
    \item{Computational aspects of combinatorics and graph theory}
    \item{Computational aspects of communication}
    \item{Computational biology}
    \item{Computational complexity}
    \item{Computational geometry}
    \item{Computational learning}
    \item{Computational Models and Complexity}
    \item{Computational Number Theory}
    \item{Cryptography and information security}
    \item{Data structures}
    \item{Database theory}
    \item{Design and analysis of algorithms}
    \item{Distributed computing}
    \item{Information retrieval}
    \item{Operations Research}
    \item{Parallel algorithms}
    \item{Quantum Computation}
    \item{Randomness in Computation}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TCS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Coding for Interactive Communication: A Survey}\\
Ran Gelles\\
ISBN: 978-1-68083-346-1\\
\\
\noindent \textit{Hashing, Load Balancing and Multiple Choice}\\
Udi Wieder\\
ISBN: 978-1-68083-282-2\\
\\
\noindent \textit{Scalable Algorithms for Data and Network Analysis}\\
Shang-Hua Teng\\
ISBN: 978-1-68083-130-6\\
\\
\noindent \textit{Communication Complexity (for Algorithm Designers)}\\
Tim Roughgarden \\
ISBN: 978-1-68083-114-6\\
\\
\noindent \textit{Quantum Proofs}\\
Thomas Vidick and John Watrous\\
ISBN: 978-1-68083-126-9

==> journaldata/TOM-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Charles Corbett}{UCLA, Anderson School of Management\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fernando Bernstein}{Duke University}
\journaleditor{Cheryl Gaimon}{Georgia Institute of Technology}
\journaleditor{Uday Karmarkar}{University of California, Los Angeles}
\journaleditor{Sunder Kekre}{Carnegie Mellon University}
\journaleditor{Panos Kouvelis}{Washington University}
\journaleditor{Michael Lapré}{Vanderbilt University}
\journaleditor{Karl Ulrich}{University of Pennsylvania}
\journaleditor{Luk van Wassenhove}{INSEAD}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TOM-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{TOMcolor}{cerise}   %new color names can be defined before use
\journalcolor      {TOMcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Technology, Information and Operations Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TOM}
\journalurl        {http://www.nowpublishers.com/TOM}
\journalissnprint  {1571-9545}
\journalissnonline {1571-9553}
\journaldoi        {10.1561/02}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Technology, Information and Operations Management publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{B2B Commerce}
\item{Business Process Engineering and Design}
\item{Business Process Outsourcing}
\item{Capacity Planning}
\item{Competitive Operations}
\item{Contracting in Supply Chains}
\item{E-Commerce and E-Business Models}
\item{Electronic markets, auctions and exchanges}
\item{Enterprise Management Systems}
\item{Facility Location}
\item{Information Chain Structure and Competition}
\item{International Operations}
\item{Marketing/Manufacturing Interfaces}
\item{Multi-location inventory theory}
\item{New Product \& Service Design}
\item{Queuing Networks}
\item{Reverse Logistics}
\item{Service Logistics and Product Support}
\item{Supply Chain Management}
\item{Technology Management and Strategy}
\item{Technology, Information and Operations in:}
	\begin{itemize}
	\item{Automotive Industries}
	\item{Electronics manufacturing}
	\item{Financial Services}
	\item{Health Care}
	\item{Media and Entertainment}
	\item{Process Industries}
	\item{Retailing}
	\item{Telecommunications}
	\end{itemize}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Technology, Information and Operations Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TOM-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Inventory Management:  Modeling Real-life Supply Chains and Empirical Validity}\\
Ton de Kok
\\ISBN: 978-1-68083-416-1
\\
\\
\noindent \textit{Operations in Financial Services: Processes, Technologies, and Risks}\\
Michael Pinedo and Yuqian Xu
\\ISBN: 978-1-68083-336-2
\\
\\
\noindent \textit{Integrated Risk Management in Supply Chains}\\
Panos Kouvelis, Ling Dong and Danko Turcic (eds.)
\\ISBN: 978-1-68083-378-2
\\
\\
\noindent \textit{Supply Chain Finance}\\
Panos Kouvelis, Ling Dong and Danko Turcic (eds.)
\\ISBN: 978-1-68083-376-8

==> journaldata/WEB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}%\raggedcolumns
\journalchiefeditor{Wendy Hall}{University of Southampton, UK}
\journalchiefeditor{Noshir R. Contractor}{Northwestern University, USA}
\journalchiefeditor{Kieron O'Hara}{University of Southampton, UK}
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Tim Berners-Lee}{Massachusetts Institute of Technology}
\journaleditor{Noshir Contractor}{Northwestern University}
\journaleditor{Lorrie Crano}{Carnegie Mellon University}
\journaleditor{Dieter Fensel}{University of Innsbruck}
\journaleditor{Carole Goble}{University of Manchester}
\journaleditor{Pat Hayes}{IHMC}
\journaleditor{James Hendler}{Rensselaer Polytechnic Institute}
\journaleditor{Arun Iyengar}{IBM Research}
%\columnbreak
\journaleditor{Craig Knoblock}{University of Southern California}
\journaleditor{Ora Lassila}{Pegasystems}
\journaleditor{Sun Maosong}{Tsinghua University}
\journaleditor{Cathy Marshall}{Microsoft}
\journaleditor{Peter Monge}{University of Southern California}
\journaleditor{Ben Shneiderman}{University of Maryland}
\journaleditor{Danny Weitzner}{Massachusetts Institute of Technology}
\journaleditor{Yorick Wilks}{University of Sheffield}
\end{multicols*}
\end{editorialboard} 

==> journaldata/WEB-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{WEBcolor}{brickred}   %new color names can be defined before use
\journalcolor      {WEBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Web Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {WEB}
\journalurl        {http://www.nowpublishers.com/WEB}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Web Science publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Agents and the Semantic Web}
    \item{Collective Intelligence}
    \item{Content Management}
    \item{Databases on the Web}
    \item{Data Mining}
    \item{Democracy and the Web}
    \item{Dependability}
    \item{Economics of information and the Web}
    \item{E-Crime}
    \item{E-Government}
    \item{Emergent behaviour}
    \item{Ethics}
    \item{Hypertext/Hypermedia}
    \item{Identity}
    \item{Languages on the Web}
    \item{Memories for Life}
    \item{Mobile/Pervasive}
    \item{Network Infrastructures}
    \item{Performance}
    \item{Privacy}
    \item{Scalability}
    \item{Security}
    \item{Semantic Web}
    \item{Social Networking}
    \item{Standards}
    \item{The Law and the Web}
    \item{The Web as an Educational Tool}
    \item{The Web in the Developing World}
    \item{Trust and Provenance}
    \item{Universal Usability}
    \item{User Interfaces}
    \item{Virtual Reality}
    \item{Web Art}
    \item{Web Governance}
    \item{Search}
    \item{Web Services}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Web Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/WEB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{An Introduction to Hybrid Human-Machine Information Systems}\\
Gianluca Demartini, Djellel Eddine Difallah, Ujwal Gadiraju and\\ Michele Catasta\\
ISBN: 978-1-68083-374-4\\
\\
\noindent \textit{Minds Online: The Interface between Web Science, Cognitive Science and the Philosophy of Mind}\\
Paul Smart, Robert Clowes and Richard Heersmink\\
ISBN: 978-1-68083-322-5\\
\\
\noindent \textit{Collective Attention on the Web}\\
Christian Bauckhage and Kristian Kersting\\
ISBN: 978-1-68083-204-4
